Temporal Graph Functional Dependencies [Extended Version]

Data dependencies have been extended to graphs to characterize topological and value constraints. Existing data dependencies are defined to capture inconsistencies in static graphs. Nevertheless, inconsistencies may occur over evolving graphs and only for certain time periods. The need for capturing such inconsistencies in temporal graphs is evident in anomaly detection and predictive dynamic network analysis. This paper introduces a class of data dependencies called Temporal Graph Functional Dependencies (TGFDs). TGFDs generalize functional dependencies to temporal graphs as a sequence of graph snapshots that are induced by time intervals, and enforce both topological constraints and attribute value dependencies that must be satisfied by these snapshots. (1) We establish the complexity results for the satisfiability and implication problems of TGFDs. (2) We propose a sound and complete axiomatization system for TGFDs. (3) We also present efficient parallel algorithms to detect inconsistencies in temporal graphs as violations of TGFDs. The algorithm exploits data and temporal locality induced by time intervals, and uses incremental pattern matching and load balancing strategies to enable feasible error detection in large temporal graphs. Using real datasets, we experimentally verify that our algorithms achieve lower runtimes compared to existing baselines, while improving the accuracy over error detection using existing graph data constraints, e.g., GFDs and GTARs with 55% and 74% gain in F1-score, respectively.

==> Algorithms/Driver.tex <==
\begin{algorithm}[tb]


\ForEach{$\sigma \in \Sigma$} 
{
    Initialize jobs $\mathcal{J}$ along with the joblets;\\
    Compute $CCost(\mathcal{J}_{ij})$ for each job;\\
    Compute $|\mathcal{J}_{ij}|$ as the number of estimated matches;\\
}
\kw{GeneralAssignment}($M_1,\dots,M_n$, $\mathcal{J}$, $CCosts$);\\
Send assigned $\mathcal{J}_{ij}$ to each worker $M_j$;\\
\If{every worker $M_i$ returns \errorsigma}
{
    \errorSigma = $\bigcup_{\sigma \in \Sigma}\mathcal{E}($\tempgraphsigma$, \sigma)$
}
\KwRet{\errorSigma};
\newline \CommentSty{/*execute at worker $M_i$*/}\\
$Joblets$:= Receive from $M_c$;\\
\ForEach{$M_j \in workers, j\neq i$}
{
    Initialize $set(edges)$ from $G_1^i$ for $M_j$\\
    Send $set(edges)$ to $M_j$
}
\ForEach{$M_j \in workers, j\neq i$}
{
    Receive $set(edges)$ from $M_j$;\\
    Merge $G_1^i$ with $set(edges)$;
}
\errorSigma := $\emptyset$;\\
\ForEach{$joblet$\ \jobletsigma $\in Joblets$}
{
    \errorSigma += \tedincremental($\mathcal{G}_T^{\sigma},\sigma)$
}
\KwRet{\errorSigma};

\caption{\kw{Driver}$($\tempgraph$,\Sigma)$}
\label{alg:Driver}
\end{algorithm}

==> Algorithms/GlobalVio.tex <==
\begin{algorithm}[tb]
%\KwIn{Relation $R$, diversity constraints $\Sigma$, and constant $k$.}
%\nonl\textbf{Procedure} \kw{LocalVio}$(F_{ij},List(\mathcal{J}_{ij}))$\\
%\tcp{To be run on each machine $M_j$}
%\nonl\textbf{Procedure} \kw{GlobalVio}$($\tempgraph$,\Sigma)$\\
%\tcp{To be run on the coordinator $M_c$}

\errorSigmaC := $\emptyset$;\\
\kw{Initialize} \hashmapX, \hashmapXY, \timehashmapX, \timehashmapXY;\\
\ForEach{Machine $M_j$}
{
    \matchesJ{i} := Receive matches from $M_j$.\\
    $\Pi_{X}' ,\pi_{XY}', \Gamma'(\Pi_{X}),\Gamma'(\pi_{XY})$:= Filter \hashmapX, \hashmapXY, \timehashmapX, \timehashmapXY \ to only contain matches from different machines than $M_j$;\\
    \errorSigmaC +=\kw{LError}$(G_{t_i},\Sigma,$\matchesJ{i}$,\Pi_{X}' ,\pi_{XY}', \Gamma'(\Pi_{X}),\Gamma'(\pi_{XY})$;
}
\KwRet{\errorSigmaC};
\caption{\kw{GlobalVio}$($\tempgraph$,\Sigma, t_i)$}
\label{alg:GlobalVio}
\end{algorithm}


==> Algorithms/LError.tex <==
\begin{algorithm}[tb]
%\KwIn{Relation $R$, diversity constraints $\Sigma$, and constant $k$.}
\errorsigma := $\emptyset$; \\
\ForEach{\matchone $\in$ \matches}
{
    \{\hashmapX, \hashmapXY\} += \matchone \\
    \{\timehashmapX, \timehashmapXY\} += $t_i$; \\
    \newtext{\permissrange := $[\kw{max}(1,t_{i}-p), \kw{min}(t_{i}+q,T)]$;} \\ 
    %\fei{this is for non-abs defn of $\rho$} \morteza{Is it OK now?} \\ 
    \If{$\{\mu_{X}(h_{t_j)}\} \setminus $ \mapfunc$\} \neq \emptyset, \forall t_j \in$ \permissrange$\}$} 
    {
        \errorsigma += $\{$(\matchone, $t_i$), (\matchtwo, $t_j$)$\}$; \\   
    }
    \ForEach{$(x.A = a) \in XY$}
    {
        \If{\matchone$.A \neq a$} 
        {
            \errorsigma += \{(\matchone, $t_i$)\}; \\   
        }
    }
}
\KwRet{\errorsigma};\\
\caption{\kw{LError}$($\tempgraph$,\sigma,$\matches$,$\hashmapX$, $\hashmapXY$, $\timehashmapX$, $\timehashmapXY$)$}
\label{alg:lError}
\end{algorithm}


==> Algorithms/alg1.tex <==
\begin{figure}[tb!]
\vspace{-1.5ex}
\begin{center}
{\small
\begin{minipage}{3.36in}
\myhrule 
\vspace{-1ex}
\mat{0ex}{
{\bf Algorithm} $\tedsingle$ \\
\sstab {\sl Input:\/} \= a temporal graph \tempgraph \ and a \tgfd $\sigma = (Q[\bar{x}],\Delta, X \rightarrow Y)$; \\
{\sl Output:\/} set of violations \errorsigma.\\

\sstab\bcc \hspace{3.6ex}\= initializes \errorsigma=$\emptyset$; \\
\icc \> set $\cal{H}$ to be all the matches of $Q[\bar{x}]$ in \tempgraph; \\
\icc\> \If $\sigma$ is constant \Then\\
\icc\> \hspace{1ex} \For\Each $h_{t_i}(\bar{x}),h_{t_j}(\bar{x})\in\cal{H}$ \Do\\
\icc\> \hspace{2ex} \If $|t_j-t_i|\in \Delta$ and $(h_{t_i}(\bar{x}),h_{t_j}(\bar{x}))\models X$ \Then\\
\icc\> \hspace{3ex} \If $(h_{t_i}(\bar{x}),h_{t_j}(\bar{x}))\not\models Y$ \Then\\
\icc\> \hspace{4ex} add $(h_{t_i}(\bar{x}),h_{t_j}(\bar{x}))$ to \errorsigma; \\
\icc\> \Else /* there exists at least one variable in $\sigma$ */\\
\icc\> \hspace{1ex} \For\Each $h_{t_i}(\bar{x}),h_{t_j}(\bar{x})\in\cal{H}$ \Do\\
\icc\> \hspace{2ex} \If $|t_j-t_i|\in \Delta$ and $(h_{t_i}(\bar{x}),h_{t_j}(\bar{x}))\models X_{constants}$ \Then\\
\icc\> \hspace{3ex} add $(h_{t_i}(\bar{x}),h_{t_j}(\bar{x}))$ to $\upsilon_X$ ,$\forall A \in X$;\\
\icc\> \hspace{1ex} \For\Each $\upsilon_{X_i} \in \upsilon_X$ \Do\\
\icc\> \hspace{2ex} compute $\upsilon_{X_iY_j}$;\\
\icc\> \hspace{3ex} \If $\upsilon_{X_i}\neq\upsilon_{X_iY_j}$ \Then\\
\icc\> \hspace{4ex} add all $(h_{t_i}(\bar{x}),h_{t_j}(\bar{x})) \in \upsilon_{X_i}$ to \errorsigma; \\

\icc\> \Return \errorsigma; \\
}
\vspace{-4ex}
\myhrule
\end{minipage}
}
\end{center}
\vspace{-2ex}
\label{alg:singleTED}
\caption{Algorithm \tedsingle} \fei{Revise to consider any single TGFD that has variables and constant literals, and uses intervals.}

\vspace{-3ex}
\end{figure}

==> Algorithms/alg1new2.tex <==
\begin{algorithm}[tb]
\KwIn{ \tempgraph,\  $\sigma = (Q[\bar{x}],\Delta, X \rightarrow Y)$.}
\KwOut{\errorsigma.}
initialize \errorsigma = $\emptyset$;\label{ln:init}\\
set $\cal{H}$ to be all the matches of $Q[\bar{x}]$ in \tempgraph;\label{ln:matches}\\


%\ForEach{entity $e \in \cal{H}$}
%{
compute $\upsilon_X$ and $\delta(X)$ for each match in $\cal{H}$;\\ 
%\fei{I don't think you need $\cal{H}$} \morteza{We need to store the matches of the graph pattern that we retrieved from the \tempgraph.}\fei{OK, it does not seem to be used nor referenced later on, and was not discussed in the text, so not sure of it's purpose.}
\ForEach{$(h_{t_i}(\bar{x}),h_{t_j}(\bar{x})) \in \upsilon_X$}
{
    compute all $\upsilon_{XY}$ and the corresponding $\delta(XY)$;\\
    \ForEach{$\upsilon_{XY}$, derived from $\upsilon_{X}$}
    {
        \If{$|\delta(XY)| \not\in \Delta$}  
        {    
        % \fei{Ques in the text about sub-intervals. Don't understand what is discarded, and what $\delta(XY) = \emptyset$ means, it always exists, unless you are doing some type of sub-interval removal.}
            discard $\upsilon(XY)$ and $\delta(XY)$;\\
        }
        \ElseIf{$Y$ is constant and $(h_{t_i}(\bar{x}),h_{t_j}(\bar{x})) \not \models Y$}
        {
        add $(h_{t_i}(\bar{x}),h_{t_j}(\bar{x})) \in \upsilon_{XY}$ to \errorsigma;
        }
    }
    \If{$Y$ is variable and $\delta(X)\neq \delta(XY)$}
    {
        /* $\delta(X)$ splits into $\delta_i(XY)$, $i\geq 2$ */\\
        add $(h_{t_i}(\bar{x}),h_{t_j}(\bar{x}))$ to \errorsigma;
    }
}
%}


\KwRet{\errorsigma};
\caption{$\tedsingle$}\label{alg:singleTED}
\end{algorithm}

==> Algorithms/incrementalTED.tex <==
\begin{algorithm}[tb]
%\KwIn{Relation $R$, diversity constraints $\Sigma$, and constant $k$.}
\errorSigma := $\emptyset$; 
\errorsigma := $\emptyset$; \\
\kw{Initialize} \hashmapX, \hashmapXY, \timehashmapX, \timehashmapXY;\\
\ForEach{$\sigma \in \Sigma$} 
{
    \kw{Initialize}(\intone) \\
    \ForEach{$t_i \in $ \intone} 
    {
        (\matches, \matchone) := \isounit($Q$, \snapshoti) \\
        \errorsigma+=\kw{LError}$($\snapshoti$,\sigma,$\matches$,$\hashmapX$,$\hashmapXY$,$\timehashmapX$, $\timehashmapXY$)$;
    } %for-t_i
\errorSigma += \errorsigma
}
\KwRet{\errorSigma};\\
\caption{\tedincremental(\tempgraph, $\Sigma$)}
\label{alg:tedinc}
\end{algorithm}


==> detection_orig.tex <==
\section{Error Detection}
\label{sec:detect}

%\fei{In addition to correctness and completeness, efficiency will be a very important factor here.  The cost of enumerating all the matches will be expensive, and optimizations are needed to make this practical.}

The error detection problem is tied to validation where we want to compute \errorSigma,  the set of violations of $\Sigma$ in \tempgraph.  Given the large scale size of \tempgraph, an error detection algorithm must be scalable and efficient.  Past work have proposed parallel scalable detection algorithms that decompose the graph patterns into connected components based on a central node with minimal radius to neighbouring nodes, and check for subgraph isomorphism around the central node in $G$.  Assuming that $G$ can be replicated or partitioned across a set of $n$ nodes, existing techniques propose strategies to distribute the matching task as evenly as possible among the nodes to maximize parallelism~\cite{fan2016functional}. 

\subsection{Overview and Challenges}
Error detection for \tgfds incur additional challenges.  Instead of retrieving matches at a single point in time, matches may occur at any  \snapshot \ for $t \in [1, T]$, and are compared pairwise $(h_{t_i}(\bar{x}),h_{t_j}(\bar{x}))$, where $|t_j - t_i| \in \Delta$, to check dependency conditions $X \rightarrow Y$.  (Without loss of generality, we assume attribute $Y$ contains a single literal $y$).  For each \snapshot, we must compute all matches of $Q$ that are isomorphic to a subgraph of \snapshot.  A naive, batch approach finds all matches for \snapshot, and then re-computes all matches for subsequent $G_{t+1}$ from scratch, for all $\sigma \in \Sigma$.   The complexity of subgraph isomorphism is known to be \npc \ for general graphs~\cite{GJ90}, making the batch approach infeasible for large graphs, and motivating the need for incremental and parallel solutions.   

Large, evolving graphs pose additional efficiency challenges over static graphs, where delta changes between snapshots need to be incorporated.  It has been shown that most graph changes affect a small portion of the graph, involving a similar set of entities.  For example, recent studies have found only 5-10\% of nodes are updated weekly~\cite{FJJ11}, and 80-99\% of the changes are highly localized~\cite{BBT18}.  In our empirical study using DBPedia, we found 82\% of updates and insertions are localized to a small set of entities.  Given this, we first take an incremental approach towards \tgfd error detection.  We avoid recomputing matches from scratch each time a change occurs, and avoid the exhaustive comparison among all matched pairs.  We build upon past work that propose  an incremental matching strategy that updates a set of matches by localizing the subgraph isomorphism operation to the induced subgraph of \snapshot \ containing only nodes within a given distance from the updated nodes~\cite{FJJ11}.  
%We introduce our incremental error detection algorithm next. 

%************* Old text about locality ***************
\eat{
\textcolor{gray}{We aim to maximize locality along three dimensions: structural, spatial, and temporal.  First, in \emph{structural} locality, we identify common subgraphs that are shared among a set of graph patterns $Q_i[\bar{x}]$.   Second, we cluster nodes among the set of graph patterns (w.r.t. a set of \tgfds) referring to the same attributes in $X$ such that we exploit \emph{spatial} locality of reference.  Lastly, we parallelize the verification task across a set of partitions according to overlapping time intervals to maximize \emph{temporal} locality. }
 In past work, relying only on structural overlap works when the graph topology remains static.  Given the evolving topology of temporal graphs, their attributes, and their values,  the \ted algorithm exploits locality along three fronts:

\begin{itemize}[nolistsep,align=left]
    \item \emph{structural locality:} \fei{Expand with more intuitive description and details.} seek pattern overlap/similarity
    \item \emph{spatial locality:} Evaluate nodes according to their shared dependency attributes to re-use matches by grouping similar \tgfds together. 
    \item \emph{temporal locality:}  Seek to process matches that occur within maximum overlapping time intervals.
\end{itemize}

%\fei{Draw algorithm/system overview, and explain main components further.}
\begin{figure}[tb]
	{\includegraphics[scale=0.47]{figures/TED.pdf}}
	\vspace{-1ex}
	\caption{\ted Overview (temporary).}\label{fig:overview}
	\vspace{-1ex}
\end{figure}
}

%that have the same matches in \tempgraph, i.e., those with embeddable patterns $Q'\subseteq Q$, overlapping literals $X' \cap X \neq \emptyset$, and overlapping time intervals $\Delta' \cap \Delta \neq \emptyset$.  By identifying these groups of related \tgfds, we decrease the time required for the matching task.  Given a set of \tgfds $\Sigma$, we introduce the notion of a \emph{summary (family?) graph} that aggregates related $\sigma \in \Sigma$ and ...\fei{complete}.  We traverse the summary (family?) graph in \tbf order to identify violations that are shared among a group of similar \tgfds.  

%**********************************************************************************************
We take an incremental approach towards error detection for a set of \tgfds and temporal graph \tempgraph.  We introduce the \emph{\uline{Inc}remental \uline{T}GFD \uline{E}rror \uline{D}etection} (\tedincremental) algorithm, which checks for errors as matches are refined to reflect changes  in \tempgraph.  We build upon the incremental matching for subgraph isomorphism algorithm, \isounit, proposed by Fan et. al.,~\cite{FJJ11}, where we incrementally check for new violations due to changes in \snapshot.  We briefly review \isounit, and then  present the \tedincremental algorithm. 

%In this section, we introduce the  \emph{\uline{T}GFD \uline{E}rror \uline{D}etection} (\ted) algorithm, that minimizes the matching overhead and maximizes re-use of retrieved matches across the dependencies. 
%We parallelize the verification task for a set of structurally similar \tgfds by distributing the workload across a set of partitions such that each partition contains matches occurring at approximately the same time interval.  Figure~\ref{fig:overview} provides an overview of \ted.  

%We first introduce necessary notions.

\subsection{Incremental Matching}
Incremental matching for subgraph isomorphism avoids recomputing matches from scratch for each \snapshot.  Let \matches \ denote the set of matches of pattern $Q$ in \snapshot, and \deltaG \ represent the changes to \snapshot \ which induce $G_{t+1}$.  The problem is to find \deltamatch, the subgraphs that are to be added or deleted from \matches \ such that $\mathcal{M}(Q,G_{t} \cup$ \deltaG $) =$ \matches $\cup$ \deltamatch.  This problem is inherently hard, with exponentially many subgraphs in \snapshot \ that may match a given graph pattern $Q$.  \isounit is a simple incremental subgraph isomorphism algorithm based on a locality property that focuses the matching task to a subgraph of \snapshot, induced by a unit change $e$ in \snapshot~\cite{FJJ11}.   

Let $d$ represent the \emph{diameter} of pattern $Q$, denoting the longest, shortest path between every two vertices in $Q$.   Recall that we consider temporal graphs of fixed nodes with insertion/deletion of an edge $e=(u_1,u_2)$, and updates to a node $u_1$.  \eat{vertex attributes.  Let denote an  to be added or removed in \snapshot \ or a node $u$ with a change in its attribute.} Let $V(d,e)$ be the set of nodes that are a distance $d$ from $e$ and \diametergraph \ be the induced subgraph consisting of nodes $V(d,e)$ and the corresponding edges.  For simplicity, we refer to edge insertions/deletions, however, updates to node $u_1$ will similarly induce a subgraph $G_t(d, u_1)$ containing nodes $d$ hops from $u_1$.  \eat{In case of an edge change (resp. attribute change), $V(d,c)$ contains all the nodes around $u_1$ and $u_2$ (resp. node $u$) within $d$ hops.} Then \changegraph \ is the result graph after applying unit update $\delta(e)$ to \diametergraph. Fan et. al., show that the changes \deltamatch \ to matches \matches, are exactly the difference between \diametermatches \ and \changematches~\cite{FJJ11}.
%Let a change $c$ be either \eat{Be careful, we have used $c$ before as constant before Ex.4, and for centre node in workload estimation. I'm not sure why we need to distinguish an update to a node as now a change $c$ is ambiguous referring to a node or an edge, and what does it mean to be a distance $d$ from $c$?} 

%\newtext{Since we consider the set of nodes to be fixed in the temporal graph, we have two types of changes, including edge and attribute changes. \cyan{Recall that \tempgraph has fixed nodes, but edges and attributes may be updated/inserted/deleted.} Firstly, let $e = (u_1, u_2)$ denote an edge to be added or removed in \snapshot. Let $V_{dhop}(u_1)$ and $V_{dhop}(u_2)$ \cyan{why not $V_d$ set of nodes $d$ hops from $e$?} be the set of nodes that are a distance $d$ from vertices $u_1, u_2$, \cyan{$e$} and \diametergraph \ be the induced subgraph consisting of nodes $V_{dhop}(u_1)\cap V_{dhop}(u_2)$ and the corresponding edges. Then,  \changegraph \ is the result graph after applying unit update $\delta$ to \diametergraph. Secondly, let node $u$ denote a node with a change in its attribute (insertion or deletion). Similarly, let $V_{dhop}(u)$ be the set of nodes within the distance $d$ of the node $u$ and build the corresponding induced graph \diametergraph. Hence, \changegraph \ is the result graph after applying the update $\delta$ to the attribute of the node $u$ in \diametergraph.  \cyan{The last 3 sentences sound redundant to what's already explained w.r.t.  $e$.} Fan et. al., show that the changes \deltamatch \ to matches \matches, are exactly the difference between \diametermatches \ and \changematches~\cite{FJJ11}.  

\isounit works by first computing the diameter of given graph pattern $Q$, and then computing \diametergraph \ from \snapshot. The algorithm then computes matches \diametermatches \ and \changematches \ by localizing the subgraph isomorphism operation to the subgraphs \diametergraph \ and \changegraph \ in \snapshot.  In the worst case, \isounit is exponential in the size of \changegraph~\cite{FJJ11}.  However, given that most graph patterns are small, the resulting diameters are also small, leading to reasonable runtimes in practice.  Furthermore, for path patterns of length $k$, and \changegraph \ that are directed acyclic graphs, we can compute matches in time $O(k! (|V_G| + |E_G|))$, where $|V_G| + |E_G|$ are the number of vertices and edges in \changegraph, respectively.  Existing techniques can be deployed, such as starting with rare labels in $Q$ and decomposing the path query into smaller queries using bi-directional search~\cite{KoschmiederL12}.  If \changegraph \ can be decomposed into a tree of width at most $k$, then we can compute matches in time $O(k! \cdot 2^k \cdot |V_G|)$~\cite{Sundaram95}.  For path queries with small $k$, this leads to feasible runtimes in practice.  Under constrained resource budgets, \isounit can be stopped at any time $t$, and matched results returned up to and including \snapshot.

%Given a temporal graph \tempgraph, it has been shown that aggregating all changes for \deltaG, for all $i \in [1, T]$ and computing subgraph isomorephism on is less efficient than processing them one at a time, due to computing subgraph isomorphism on smaller graphs (albeit more frequently)~\cite{FJJ11}.  We remove redundant changes and then apply \isounit, and aggregate the matches for each of \diametermatches \ and \changematches to compute \deltamatch.

%\begin{example}
%\fei{Give example showing execution of \isounit.}
%\end{example}


\subsection{Incremental Error Detection}
\label{sec:incdetect}
Consider $\sigma \in \Sigma$, where $\sigma=(Q[\bar{x}],\Delta,X \rightarrow y)$.  Let \errorsigma \ be the set of violations of $\sigma$ in \tempgraph, where \errorSigma $ = \cup_{\sigma \in \Sigma}$ \errorsigma.  To determine whether \errorsigma \ is empty, we compute match \matchone \ in \snapshot, and compare it against all matches \matchtwo, where $|t_j - t_i| \in \Delta$.  Since matches are computed starting at $G_1$, and incrementally updated for each subsequent snapshot, a naive strategy compares the current \matchone \ against all computed matches \matchtwo \ for $j > i$, until $i = (|T|-p)$.  For the current \snapshot, this requires at least $(|T|-p) \cdot$ \kw{min}$(q, |T|-(i+p)+1)$ pairwise comparisons, and storing all matches from \snapshoti, and from snapshots $\{G_{t_{i+p}}, \ldots , G_{t_{i+q}}\}$.  \eat{Figure~\ref{}\tbf \fei{Morteza: please draw corresponding window of matches for a given $G_i$ w.r.t. $\sigma$.} shows the space of pairwise comparisons where the blue X's indicate the current $t_i$ for \matchone, and the intervals represent snapshots where the corresponding match \matchtwo \ may occur.}  There are $(|T|-p)$ and \kw{min}$(q, |T|-(i+p)+1)$ snapshots where \matchone \ and \matchtwo \ can occur, respectively. 

\tedincremental is an incremental detection algorithm for TGFDs that avoids having to save past matches and reduces the exhaustive number of pairwise match comparisons to set difference operations bounded by the domain of the consequent literal $l$ in $\sigma$.  For each $\sigma \in \Sigma$, \tedincremental \ incrementally computes all matches \matchone \ for each \snapshoti \ (using \isounit), and adds each \matchone \ to a hashmap of observed values w.r.t. $X$ and $Y$ for all snapshots $\{G_{t_1}, \ldots, $ \snapshoti$\}$ evaluated thus far.  If \matchone \ shares the same values in $X$ as another match \matchtwo \ but with different values in $Y$, where $|t_j - t_i| \in \Delta$, then \matchpair, and their timestamps $(t_i, t_j)$ are added to \errorsigma.  Let a violation \vio represent a pair of matches \matchpair $\not \models \sigma$, and their timestamps, i.e., \vio $=\{$\matchpair, $(t_i, t_j)\}$.  Let \intone and \inttwo represent the time intervals where matches \matchone \ and \matchtwo \ are found, i.e, the time range of matches for $\sigma$.  The allowable time difference between \matchone \ and \matchtwo\  is defined by $\Delta$, and the scope of \inttwo will necessarily depend $t_i$, the time of \matchone.  We define \intone and \inttwo as follows, 

\vspace{-0.6cm}
\begin{equation} \label{eqn:intervalbounds}
\begin{split}
\intone & = [t_{1}, t_{|T|-p}] \\
\inttwo & = [(\matchonetime + p), \matchtwotime'], \texttt{where } \matchtwotime' = 
\left\{
    \begin{array}{l}
      T,  (\matchonetime + q) > T \\
      (\matchonetime + q), o.w.
    \end{array}
\right.
\end{split}
\end{equation}
\vspace{-0.6cm}

For a retrieved match \matchone \ occurring at $t_i$, let \permissrange \ be the time range of all matches \matchtwo, $t_j \in $ \permissrange,  such that $|t_j - t_i| \in \Delta$.  We call \permissrange \ the \emph{permissable range} of \matchone.  Intuitively, \permissrange \ defines the time scope of matches for comparison against a given \matchone.  To avoid enumeration of all pairwise matches in the permissable range of \matchone, we define a hash map, \hashmapX$(t_i)$, that partitions all matches of $Q$ according to their values in $X$, and records the observed values in $X$ for all retrieved matches up to and including $t_i$.   Specifically, let \hashmapX $= \{$\matchtwo $|$ \matchone$.A =$ \matchtwo.$B, \forall$ (\matchone$.A$, \matchtwo.$B) \in X, j \leq i\}$. We simply use \hashmapX \ when $t_i$ is clear from the context.   We can sub-partition the matches in \hashmapX \ according to shared values in $X$ and $Y$.  Let \hashmapXY \ denote the set of matches with equal values in $XY$, such that \hashmapXY $\in$ \hashmapX.  To capture the time occurrence of these matches, we define \timehashmapX \ to contain the timestamps when the corresponding matches in \hashmapX \  occur, i.e., \timehashmapX = $\{t_j | $\matchtwo \ $ \in $ \hashmapX $\}$.  We define \timehashmapXY \ in a similar manner.  To determine which partition a given match \matchone \ belongs, let \mapfunc\ denote the function that returns the corresponding \hashmapXY, i.e., \mapfunc = \hashmapXY \ such that \matchone\  $\in$ \hashmapXY.

\begin{example} \label{exmp:IncTED_def}
%\fei{Fill in example showing above notions corresponding to the motivating example, i.e., pick one of the domain examples and show consistent cases and error cases with \hashmapX, \hashmapXY, \timehashmapX, etc.}
Recall $\sigma_1$ from Example~\ref{exm:tgfdDefinition}, where matches with patient \lit{Jack} occur at $\{t_1, t_3, t_6, t_8\}$. We then have \hashmapX $=\{h_{t_1}(\bar{x}), h_{t_3}(\bar{x}), h_{t_6}(\bar{x}), h_{t_8}(\bar{x})\}$ with \timehashmapX$=\{t_1, t_3, t_6, t_8\}$. 
Similarly, we define \hashmapXY$=\{\{h_{t_1}(\bar{x}), h_{t_3}(\bar{x}), h_{t_6}(\bar{x})\} \{h_{t_8}(\bar{x})\}\}$ with the corresponding timestamps \timehashmapXY$=\{t_1, t_3, t_6\} \{t_8\}$.
%Going back to Figure~\ref{fig:mainExample} and $\sigma=(Q_1[\bar{x}], \Delta_1=(2,3\ hours), [x.name=x.name \land z.name=`$\lit{Covid-19}'$] \rightarrow [y.name=y.name])$, then \hashmapX$=\{[$\lit{Jack}, \lit{Covid-19}$]\}$ with \timehashmapX$=\{t_1,t_3,t_6\}$. Similarly, \hashmapXY$=\{[$\lit{Jack}, \lit{Covid-19}, \lit{remdesivir}$], [$\lit{Jack}, \lit{Covid-19}, \lit{dexamethasone}$]\}$ with the corresponding timestamps \timehashmapXY$=\{[t_1,t_3], [t_6]\}$.}
\end{example}

\stitle{Algorithm.} For each $\sigma \in \Sigma$, \tedincremental computes matches of $Q$ in \snapshoti \ at each $t_i \in $ \intone \ using \isounit.  For a new match \matchone, we add \matchone \ to \matches, and to the set of matches \hashmapX \ and \hashmapXY \ sharing the same values in $X$ and $XY$, respectively.  We also add $t_i$ to \timehashmapX and \timehashmapXY \ to capture the times when these matches occur.  Insertions, updates or deletions may occur from the previous snapshot to derive the current \snapshoti.  If a change in attribute value $A \in XY$ induces a new match, we perform the same updates to \matches, \hashmapX, \timehashmapX, etc.  If there is no change to a previously identified match, we then assume that the match persists from the previous time stamp, and we simply add $t_i$ to \timehashmapX \ and \timehashmapXY.  If an edge $e$ induces a match to be deleted, then no update is made.   

To verify whether a new match \matchone \ causes a violation, we must check whether there exists matches \matchtwo \ in the permissable range of \matchone \ that: (1) share the same values in $X$, but with a different value in $Y$; or (2) in the case of constant literals, whether the values in \matchone \ are equal to the given constant literals in $X$ and $Y$.  In the first case, to achieve consistency, we require $\forall t_j \in \rho(t_i)$, \mapfunc = $ \mu_{X}(h_{t_j})$.  If this condition is false, then there exists at least one match \matchtwo, which together with \matchone, $j < i$, causes a violation, i.e., $\exists t_j \in \rho(t_i)$, \mapfunc $\neq  \mu_{X}(h_{t_j})$.  If this occurs, then we add (\matchone, $t_i$) and (\matchtwo, $t_j$) to \errorsigma.  In the second case, for each given constant literal $x.A = a$ in $X$ (or $Y$), with constant $a$, we check whether \matchone$.A = a$.  If not, then we add (\matchone, $t_i$) to \errorsigma.
\tedincremental makes one pass over all $t \in [1,T]$ and checks matches at the current $t$ against all previously seen matches.  Once a match has been evaluated, it is discarded while its observed values in $X$ and $Y$ are maintained in \hashmapX \ and \hashmapXY, respectively. \tedincremental avoids having to compare all pairwise matches as the computation of \errorsigma \ can be done by checking whether the set difference between the partitions containing matches \matchtwo, $\forall t_j \in$ \permissrange, and the partition containing \matchone, is non-empty.  If so, then all the matches occurring at $t_j$ lie in the permissable range of \matchone, and share the same value in $X$ but with a different value in $Y$.  Specifically, \errorsigma = $\{$(\matchone, $t_i$), (\matchtwo, $t_j$) $| \{\{\mu_{X}(h_{t_j)}\} \setminus $ \mapfunc$\} \neq \emptyset, \forall t_j \in$ \permissrange$\}$.
Algorithm~\ref{alg:tedinc} provides \tedincremental details. 

\input{Algorithms/incrementalTED}

\input{Algorithms/LError}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[t]
\begin{figure}[tb!]
    \centering
    \includegraphics[scale=0.32]{figures/IncTED.png}
        \vspace{-0.3cm}
    \caption{\tedincremental algorithm.}  
    %\fei{Replace with my comment below. I would use this figure to show how matches are computed incrementally and how the $\Pi,\pi, \Gamma$ structures are maintained along with a temporal graph of matches to show how the error set is computed.}
    \label{fig:IncTEDPermissable_range}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{example}
%\fei{Morteza: show visual example \tedincremental execution as per the Algorithm description continuing previous example.  How are updates considered at each iteration.}
Recall $\sigma_1$ and its matches, as shown in Figure~\ref{fig:IncTEDPermissable_range}, along with the \permissrange, and \mapfunc = \hashmapXY \ values for each match \matchone. We check for errors between $h_{t_1}(\bar{x})$ and $h_{t_3}(\bar{x})$ where $t_3 \in \rho(t_1)$ by computing \{$\mu_{X}(h_{t_3}(\bar{x})) \setminus \mu_{X}(h_{t_1}(\bar{x}))$\} = $\emptyset$; hence, there exist no errors.  However, $t_8 \in \rho(t_6)$, and $\{\mu_{X}(h_{t_8}(\bar{x})) \setminus \mu_{X}(h_{t_6}(\bar{x})) \} = h_{t_8}(\bar{x})$, reflecting an inconsistency in medications \lit{remdesivir} and \lit{Dexamethasone} at $t_6$ and $t_8$, respectively.   
\eat{
\newtext{Continue with Example~
\ref{exmp:IncTED_def}, we show the permissable range of each match in Figure~
\ref{fig:IncTEDPermissable_range}, \emph{e.g.,} $\rho(t_1)=\{t_3,t_4\}$, $\rho(t_3)=\{t_5,t_6\}$, $\rho(t_6)=\{t_8,t_9\}$ and $\rho(t_8)=\{t_{10},t_{11}\}$. We next compute $\mu_{X}$ for the matches, where we have $\mu_{X}(h_{t_1}(\bar{x}))$, $\mu_{X}(h_{t_3}(\bar{x}))$ and $\mu_{X}(h_{t_6}(\bar{x}))$ are the same and different than $\mu_{X}(h_{t_8}(\bar{x}))$. However, $t_8 \in \rho(t_6)$ but $\mu_{X}(h_{t_8}(\bar{x})) \cap \mu_{X}(h_{t_6}(\bar{x}))=\emptyset$, which leads us to consider the matches at $t_6$ and $t_8$ as violations.}  
}
%\fei{The benefit of this method as highlighted in blue in the paragraph above is that we don't have to do all pairwise matches.  Can you please show this via the example, where we compute the set difference, show partitions, permissible ranges, and exactly how the error set is computed based on the explanation of the blue text.}
%\fei{Please replace Figure 2 with a new figure showing all the structures and their values for the Jack example from Figure 1. For each match at $t_3, t_6, t_8$ explain what happens to the structures, and how the error at $t_8$ is found.}
\end{example}


\stitle{Runtime Complexity.}  The runtime of \tedincremental is dominated by \isounit.  This graph pattern matching is inherently exponential in the size of \changegraph. \eat{taking $O(2^{|V_{\delta(e)}|})$ time, where $|V_{\delta(e)}|$ are the number of edges in \changegraph.}  Given that $|Q|$ is normally small, leading to small $d$ and \diametergraph, it is unlikely to find an exponential number of subgraphs isomorphic to \changegraph~\cite{FJJ11}.  However, when changes involve edge or attribute insertion/deletion, matches may be added or deleted.  We can achieve a tighter complexity bound if we maintain a list of approximate matches \approxmatches, that are just short of an edge to qualify as a match of $Q$ in \changegraph.  We can then compute matches by iterating over \approxmatches \ for each change, leading to time $O(|$\approxmatches$| \cdot |\texttt{changes}||$. As mentioned in Section~\ref{sec:incdetect}, this matching complexity is reduced for path queries over DAGs.

For each $\sigma \in \Sigma$, validating the literals at each $t_i$ depends on the number of matches, and the size of the permissable range of \matchone \ at $t_i$.  The number of matches is bounded by the attribute domain of literals in $XY$, which we denote as $|dom(XY)|$.  The permissable range is upper bounded by $|T|$.  Hence, validation of $\Sigma$ can be done in $O(|\Sigma| \cdot |dom(XY)| \cdot |T|)$.  %\fei{abuse of notation for attribute values in literals.}

%To compute \errorSigma \ for a set of \tgfds $\Sigma$, matching and verification dominate the runtime, which requires enumerating all matches $(h_{t_i}(\bar{x}),h_{t_j}(\bar{x}))$ for each $\sigma \in \Sigma$.  

%\subsubsection{Stable Time Intervals}
%\fei{Add new section in preliminaries about TGraph and temporal graph evolution model.  Expand upon the preliminaries here and how the validity period and other properties are useful for inconsistency detection.}
%In a temporal graph \tempgraph, changes occur in structure, attributes, and values representing evolution of the graph.  We associate each change with a timestamp.  Similarly, when the topology and values do not change, specific attribute values exist over a range of time points.  We can coalesce these time points to define a \emph{stable time interval}, $\delta$, representing the time points when particular values exist in \tempgraph.  As introduced in Section~\ref{sec:prelim_graphs}, the interval model captures this intuition to represent evolution in graphs. Henceforth, we assume such an interval exists denoting time periods where specific attributes and values hold continuously over the interval.

%For error detection w.r.t. a \tgfd $\sigma=(Q[\bar{x}],\Delta, X\rightarrow Y)$, we must verify whether the values in $X$ functionally determine the values in $Y$.  Hence, for each unique combination of values in $X$ ($Y$), we have an associated interval $\delta(X)$ ($\delta(Y)$) representing the time points where values in $X$ ($Y$) exist in \tempgraph.  Recall, without loss of generality, $\sigma$ is in normal form.

%This period of stability $\delta$, where the topology and attribute values do not change, can be captured by coalescing the time points where shared values in $X$ (and $Y$) occur.  
\eat{For a given $\Delta$,  matches satisfying the pattern $Q$, and values that are equal in $X$ over a time period $j \in T$, the values in $Y$ should be equal, $j \in \Delta$.} 

%Intervals provide a compact representation of shared topology, values and semantics, where changes elicit the creation of new time intervals.  For example, \lit{Gareth Bale's} change in nationality is modeled via two different intervals, capturing a change from temporary to permanent status.  Recent work such as \tbf~\cite{HT14}, and \emph{TGraph} utilize intervals to model evolution in topology, vertex and edge attributes~\cite{MS17}.  A time interval $[s_1,s_2]$ represents a set of time points.  A TGraph is represented using  temporal relations, correlating the existence of a vertex or edge, and an assignment of a value to a vertex or edge attribute, to a time interval.  By using such an interval representation, for a given graph pattern $Q[\bar{x}]$, a set of attributes $X, Y$, and their values, we can identify the time periods where the values hold.  For a match $h(\bar{x})$ associated with an interval $[s_1,s_2]$, we assign the time points $t_{s_1}$ and $t_{s_2}$ to $h(\bar{x})$, and check whether the interval is within $\Delta$ i.e., $|h_{t_{s_2}}(\bar{x}) - h_{t_{s_1}}(\bar{x})| \in \Delta$.

%**********************************************************************************************


==> learning.tex <==
\section{Learning from Changes and Errors}
\label{sec:learn}

To perform temporal object matching and reconcile entities, we can use the graph patterns that are embedded within a pattern, at and look at the errors at about the same point in time.  Entities that share overlap for a long period of time can be linked, and looking at changes (errors) can also give clues.

\fei{
\begin{enumerate}
    \item Can we quantify the deviation of these changes and errors to derive an ordering?  Consider the use of influence functions and the influence of values and errors.
    \item By learning from the overlap of matches and overlap among graph patterns $Q$, can we infer relationships among the error values if their deviations are less than a given $\epsilon$?  For example, matches in \tempgraph that satisfy players and coaches may share significant overlap.  Similarly, their corresponding \tgfds may also share overlap in their graph patterns.  Based on this input data, can we infer relationships among their changes/errors?   An error w.r.t. the player \tgfd may be due to a new record satisfying the coach \tgfd.  Similarly, this can be extended if we have subsequent manager to owner \tgfds that can be defined. 
    \item Possible cost metrics: (i) quantify notion of stability thus far, up to the time of error; and (ii) magnitude of change relative to others or itself in the past.
    
\end{enumerate}

}


==> oldmodel.tex <==
%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$

\subsection{Workload Model and Estimation - Model2}\label{sec:workloadAndEstimation2}

%Before explaining the description of the \tedparallel algorithm, we provide some definitions.


Consider a set of $n$ worker machines $M_1 \ldots M_n$, and a coordinator machine $M_c$.  A fragmentation of \tempgraph \ across the machines is a set of fragments \fragments, each a subgraph of snapshot $G_i$ on machine $j$, where $i \in [1, T], j \in [1, n]$.
Given $\Sigma$ and a fragmentation \fragments, we compute \errorSigma \ in parallel such that the workload assignment across the $n$ machines is distributed as evenly as possible, and the communication cost between the machines is minimized.  

Towards this objective, it is important to accurately estimate the number of matches for query pattern $Q$ for each $\sigma \in \Sigma$.   We compute the expected workload by estimating the number of subgraph matches for each $\sigma \in \Sigma$.  Since a given fragmentation may split a match of $Q$ \ w.r.t. $\sigma$ across two or more machines, we estimate the data that must be copied between machines to compute a match, as the communication cost.  Each machine $M_j$ locally computes the matches against $F_{ij}$, and performs local validation w.r.t. $\sigma$ to compute \errorsigmaj, and then sends the matches and errors to $M_c$.  Changes to \fragment \ are sent to $M_j$, which may add or remove  inconsistencies from \errorsigmaj \ and \errorsigma. Lastly, edge insertions/deletions and attribute updates can lead to workload imbalance across the machines where selected machines incur an increasing burden of the workload. If the processing time at any machine lies beyond the given lower and upper bounds, then we re-balance the workload via a new workload assignment~\cite{aggarwal2003load}. 


Before explaining the description of the \tedparallel algorithm, we provide some definitions.

\eat{
\begin{definition}
Given two snapshots $G_i$ and $G_j$, $\delta_{i,j}(G_i,G_j)$ contains all the differences between $G_i$ and $G_j$ including: edge insertion and deletion, node attribute insertion and deletion.
\end{definition}

\begin{definition}
Let $G_{i}^j$ represent the subgraph of $G_i$ on machine $j$.
Let $\{F_{i1},\dots,F_{in}\}$ be a set of \emph{fragments} of \tempgraph \ at timestamp $i$, 
where each fragment $F_{ij}$ = \{$G_1^j$, \snapshotdiff{1}{2}{G_1^j,G_2^j}, \dots, \snapshotdiff{(i-1)}{(i)}{G_{i-1}^j,G_{i}^j}\}. A fragment $F_{ij}$ is located at machine $j$.
\end{definition}
}

\begin{definition}
Consider a \tgfd $\sigma=(Q[\bar{x}],\Delta, X \rightarrow Y)$ and $v_{\hat{c}}$ as a center node with minimum radius in $Q$, where \emph{radius} is the longest shortest path between $v_{\hat{c}}$ and any node in $Q$. We define $Candid(\sigma,F_{ij})=\{v_1,\dots, v_k\}$ as a set of candidate nodes in $F_{ij}$ that are from the same type of $v_{\hat{c}}$ \emph{i.e.,} $L(v_{\hat{c}})=L(v)$ for all $v\in Candid(\sigma,F_{ij})$.
\end{definition}  


\eat{\begin{definition} (\emph{joblet}) 
A joblet  is defined based on the nodes in $Candid(\sigma,F_{ij})$ for each fragment $F_{ij}$ and each \tgfd $\sigma \in \Sigma$. A joblet represents a \emph{work unit} in our distributed setting. More specifically, for a given \tgfd  $\sigma=(Q[\bar{x}],\Delta, X \rightarrow Y)$ and a fragment $F_{ij}$, $\mathcal{J}=(\sigma,v,F_{ij},G(v,d))$, where (a) $\sigma$ is the corresponding \tgfd; (b) $v$ is a candidate node in $Candid(\sigma,F_{ij})$; (c) $F_{ij}$ is the fragment that contains $v$; and (d) $G(v,d)$ is the induced subgraph $d$-hops around node $v$, where $d$ is the diameter of $Q$. 
Let $W_{ij}(\Sigma,$ \tempgraph) be all the joblets aggregated for $F_{ij}$ and $W(\Sigma,$ \tempgraph) be the aggregation across all $j$.
Since we have a fixed set of nodes in \tempgraph, the total number of joblets is fixed and is independent of the timestamps.
\end{definition}
}


\begin{definition} (\emph{joblet}): Given a \tgfd  $\sigma=(Q[\bar{x}],\Delta, X \rightarrow Y)$,
let $\mathcal{J}(\sigma,F_{ij}, \mathcal{G}(v',d))$ \ represent a \emph{joblet} denoting a unit of work to compute matches of $\sigma$ on fragment $F_{ij}$ over \tempgraphk = $\{G_1(v',d), G_2(v',d), \ldots , G_{i}(v',d)\}$, $v' \in Candid(\sigma,F_{ij})$ \ such that $\forall s, s' \leq i, |s' - s| \in \Delta$.  The fragment \fragment \ contains node $v'$, and \tempgraphk \ are the induced subgraphs $G_t(v',d)$ $d$-hops around $v'$ for diameter $d$ of $Q$ for $t \leq i$. Let \jobletSigma \ represent jobs for a set of \tgfds $\Sigma$,  i.e., $\cup_{\sigma \in \Sigma}$ $\mathcal{J}(\sigma,F_{ij}, \mathcal{G}(v',d))$ 
\end{definition}

Intuitively, \tempgraphk \ are the induced subgraphs from \tempgraph \ that must be checked to compute the matches to $Q$.


%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$%$


 We estimate the size of a joblet $\mathcal{J}(\sigma,F_{ij}, \mathcal{G}(v',d))$ at timestamp $i$ as the size of the induced subgraph, counting the number of edges, that we must evaluate to validate $\sigma$. 

\begin{equation} \label{eq:unitworkload}
    |\mathcal{J}(\sigma, F_{ij},G_i(v',d))|=|G_i(v',d)|^{|Q|}
\end{equation}

Similarly, for \jobletSigma, we sum all joblets across all $\sigma \in \Sigma$ on machine $M_j$ and for \totalworkload, we sum all joblets across all machines..
\eat{, $|G(d,v)|$ (resp. $|Q|$) is the size of the induced subgraph graph (resp. size of the pattern of $\sigma$) in terms of the number of edges. $|\mathcal{J}|$ gives us an estimation of the amount of work needs to find the matches of $\sigma$, where we need to enumerate the subgraph $G(v,d)$ and find the matches.} Since the matching part is done sequentially, the expected runtime will be exponential to the size of $Q$ in the worst case. 


%\fei{I think you can merge Eqn(2) and (3) together by defining a joblet to be the number of nodes/edges of the induced subgraph $d$-hops around node $v$, where $v$ is contained in fragment $F_j$.}  
%\fei{If you want to consider the specific time of a fragment then add $F_{j}^i$.  The workload for a machine $W_j(\Sigma,$\tempgraph) is simply all the joblets aggregated for a specific $F_j$.  Then total workload is just aggregation across all $j$.}

%\fei{Why are there 3 different definitions of Workload?  Isn't workload across all machines $W(\Sigma, G_T)$ and over each machine it's $W_j(\sigma, F_j)$ for those $\sigma \in \Sigma$ that can be matched on $F_j$? I recommend you aggregate eqn (2) and (3) together as suggested with the previous comment.  Eqn (4) is just an aggregation over all machines (to make this more general) and avoid having another workload discussion later on how to deal with changes.} \morteza{Revised.}
%%%%%%%%%%%%%%$Candid(\mathcal{G}_T, \hat{u}, d)$ is a \emph{bag} of candidate nodes (may contain duplicates) that initially contains all the nodes of the same type $L_1(\hat{u})$ in $G_1$. Moreover, for any subsequent difference $\delta_{i,j}$, if there exists a change within $d$ hops of a node $v$ in $Candid(\mathcal{G}_T, \hat{u}, d)$, we add $v$ again to the bag. 
%%%%%%%%%%%%%%$|G_1(d,v)|$ (resp. $|Q|$) is the number of edges of the induced subgraph within $d$ hops of the node $v$ in the snapshot $G_1$ (resp. pattern). Equation~\ref{eq:workload} looks at the size of all the possible subgraphs in \tempgraph that are potential matches of $Q$ to compute the workload of $\sigma$. Since subgraph isomorphism exponentially grows in terms of the graph and pattern size, we compute the runtime using the exponential formula in Equation~\ref{eq:workload}. Similarly, we define $W(\Sigma,$\tempgraph$)=\bigcup_{J \in Joblets}W(J)$ as the total amount of workload.


%\fei{OK, I get the idea.  We discussed changing Eqn(2) to be defined w.r.t. $G_1$ (same function) and then considering the induced subgraph around the number of \emph{changes}.  The current function looks like you re-do the computation for each \emph{snapshot} which looks very expensive.} 

%\morteza{I changed the formula to only look at $G_1$ to compute the subgraph size, but consider the changes in $\delta_{i,j}$ as well.} 

%\fei{Can you please be specific where $\delta_{i,j}$ is considered in Eqn(2)?  Based on our June 2 discussion, this has to now consider the induced nodes that are matched by the edge insertion/deletion.}

%\fei{From our May 28th discussion, there were several re-organization comments, assumptions to be listed (replication, changes going to all nodes, why is this reasonable?), and details of the complete parallel model you envision to be explained. Please elaborate on the more general no-replication case, similar to the GFD paper where replication is considered to be expensive and not possible.  Is this what you intend to do?  Explain why or why not.} 
% \fei{What is the relationship between nodes $u, v$?  It seems you are applying this exponential enumeration for each induced subgraph at each snapshot (for each timestamp).  Why not do it once for $G_1$ and then apply the incremental matching algorithm isounit to just look around $d$-hops from the changed edge from the existing matches at $t_1$?}

%\newtext{\stitle{Workload estimation.} Given a \tgfd $\sigma=(Q[\bar{x}],\Delta,X\rightarrow Y)$ and a temporal graph \tempgraph, procedure \tbf estimates the workload of $\sigma$ (\workloadsigma) as follow: (1) It first finds the center node $\tilde{c}$ \cyan{why tilde?} of the pattern $Q$ with the minimum radius $r$. (2) It finds the set of candidate matches of $\tilde{c}$ ($Candid(\tilde{c})$) in the first timestamp $G_1$ of \tempgraph. A node $v \in Candid(\tilde{c})$, if it has the same type as $\tilde{c}$ ($L_1(v)=L(\tilde{c})$).  \cyan{Why would it not have the same type?  Is this not checked during the candidate matching?} (3) For each node $v \in Candid(\tilde{c})$, we compute $|G_1^r(v)|$ as the number of edges of the subgraph centered on $v$ with $r$ hops. \cyan{d-hops, if you are computing a subgraph centered on $v$ within $d$ hops, may want to define the vertices first, and then count the edges from this subgraph. } This can be done using Breadth-first search (BFS) algorithm starting with $v$. (4) Finally, for each node $v \in Candid(\tilde{c})$, we compute the workload as $|G_1^r(v)|^{|Q|}$, where $|Q|$ is the size of the pattern (number of edges) and sums up the workload of all the nodes in $Candid(\tilde{c})$ as \workloadsigma. \cyan{suggest you define the workload function as a formula first, and then explain.  It sounds like you are computing an induced subgraph, $d$-hops away from $c$, counting the edges in this subgraph. Explain why this is a good workload estimation formula.}  We only look at the first timestamp $G_1$ to estimate the workload as per our assumption that the temporal graph \tempgraph \ will have few changes across timestamps compare to $G_1$.}
\subsubsection{Communication Cost}
To estimate the communication cost, we estimate the amount of data that must be transferred from one machine to another.  For a query pattern $Q$, a fragment $F_{ij}$ may only contain a partial match, i.e., some nodes and edges that match $Q$ reside in another machine $M_{j'}, j \neq j'$.  We estimate the communication cost \ccost \ as, 

\begin{equation} \label{eq:datashipment}
    CCost(\mathcal{J},M_j)=\sum|e(u_1,u_2)\in G(v,d)| \ \mid (u_1\not\in F_{ij} \lor u_2\not\in F_{ij})
\end{equation}


\begin{example}
\fei{Show picture example of parallel machines, fragments across machines, joblets, and how partial match can occur, and the communication cost.}
\end{example}

Equation~\ref{eq:datashipment} estimates the data shipment in terms of the number of edges for a given joblet along with its machine assignment. It counts the number of edges in the induced subgraph that has (at least) one end point not reside in $F_{ij}$. 
%This function will be used in the coordinator $M_c$ for the first snapshot $G_1$ as we later send updates of the following snapshots (difference files $\delta_{i,j}$) to the workers.

\eat{\fei{I think there are two elements to CC: (1) initial data shipment of subgraph nodes/edges from machine $M_j$; and (2) $M_j$ sends matches to $M_c$ to do pairwise comparisons (either incrementally or at the end).}
\morteza{We have talked about this before (mainly number (2)) as it is impossible to estimates the number of matches that we need to send to $M_j$. This cannot be calculated unless the workers find the matches. However, you asked to keep this comment and we discuss more with Yinghui.}
\todo[inline]{Reply? What about incremental data shipment due to changes?  New edges that match but reside in a different machine?  How is CCost computed for incremental changes?  Why do we not consider (2) above?  Justify.}

\morteza{After sending the updates to the workers for the new timestamp, the coordinator also sends a list of nodes/edges that has to be shipped from $M_j$ to all other workers. This list will be computed after each superstep (snapshot).  \fei{At this point, it's possible that the time cost and the CCost have changed since the last iteration.  We would have to estimate the change in workload/joblet to know how much. } The CCost() is computed based on the current job assignment, where we haven't processed the next timestamps yet. How do we include future changes of the current snapshot in the CCost()?  \fei{We can only estimate based on the changes we currently have.  If the change in workload (joblet size) has changed "a lot", then we may also lose 2-approximation of the GA if the times fall out of bounds.  Pls confirm if my undertanding is correct: we use the GA alg. to derive a schedule that can guarantee 2T, but then lose that guarantee if changes arrive, and then have to re-do GA to re-gain the 2T time based on burstiness detection?}\morteza{Yes. this is correct. Previously, I was trying to maintain the size of all joblets when the changes are about to send. This can be done for free. One way to tackle this issue would be to check if 2T is still guaranteed or not, and whenever it is not, we trigger the re-balance procedure. What do you think?}  
\fei{I think we need to think about how to estimate the impact of incoming changes via change in $|G(v,d)|$ and whether new edges that are introduced incur higher \ccost to maintain this 2T time approximation.  It is a weak point to say we use a GA alg that can have these guarantees if we don't maintain them or at least try to.  The time will toggle from an upper bound of 2T to something beyond, and then we have to incur a high overhead to re-assign to re-gain the 2T again.  The performance of the parallel algorithm cannot be bounded by the 2T statement.  } OK, I see what you mean.

We calculate the CCost() each time we need to do re-balancing.  \fei{Assuming you only re-compute the GA after re-balancing.} To justify that, I would say this CCost() is computed based on the current joblet assignment and it is the amount of edges needed to be shipped to other fragments. For the future changes, we might re-assign joblets based on the bustiness detection, and we will re-compute it again if needed.} \fei{this entire description of how the algorithm works in light of changes needs to be visualized.  A lot of this is lost in the text and not clear.}
}


\stitle{Remark.} We assume that the coordinator $M_c$ maintains a location map $\mathcal{L}$ of the machine locations where each induced subgraph $G(v,d)$ resides at a given time $t_i$.  At time $t_{i+1}$, $M_c$ sends attribute updates and edge insertions/deletions to the latest machine according to $\mathcal{L}$.

%fei: summarized to make the main point and avoid redundant statements
\eat{Sending updates to workers. As we continue in time, updates are coming to the graph in the difference files. $M_c$ needs to send these updates to the right machine in order the machines update their matches incrementally. Assume  a joblet $\mathcal{J}=(\sigma,v,F_{ij},G(v,d))$ is assigned to $M_j$ and all the nodes/edges in $G(v,d)$ are already shipped to $M_j$ at timestamp $i$. We maintain a list in the $M_c$ contains the nodes/edges of $G(v,d)$ along with $M_j$ as their current location. For the next timestamp $i+1$, if an edge is added to/removed from $G(v,d)$, $M_c$ sends the update to $M_j$ as the latest location of $G(v,d)$. Similarly, if an attributes has changed in $G(v,d)$, $M_c$ sends the update to $M_j$. Using this technique, $M_c$ is able to send the next timestamps to the corresponding workers for incremental matching. }

%%%%%%%%%%%%%%\newtext{\textbf{Remarks.} The workload and communication cost are computed in the coordinator and we assume the coordinator has full view of the temporal graph \tempgraph. There also exists a fixed communication cost for the $M_c$ to send $\delta_{i,j}$ to the workers. \fei{this last stmt is no longer true.} To minimize this cost, $M_c$ will only send relevant changes to the workers based on the joblet assignments. A change (\emph{i.e.}, edge insertion/deletion or attribute insertion/deletion) is relevant to a joblet, if the types of all the involved nodes in the change exist in the \tgfd of the joblet.}

%\fei{ [DISCUSSION POINT]
%\begin{enumerate}  
%    \item So this is assuming you replicate the nodes that a machine, say $M_1$ needs from $M_2$, right?   So $M_1$ has some of $M_2$'s nodes, and all subsequent changes involving those nodes (and edges) are sent to $M_1$ and $M_2$?  If so, this needs to be stated as people will think how future changes are handled when you have disjoint fragments, when this is not what we are handling.
%    \item My 5th point in Section 6.1: how are future edge insertions or node attribute changes handled that may induce a new match after $t_1$?  E.g., A node changes their name attribute at $t_3$.  Is it possible to consider communication cost due to changes after $t_1$? Is there some restriction?  Given the changes, can we estimate which matches are affected, in the neighbourhood of the focus node to estimate communication cost for $t > t_1$?
%\end{enumerate}
%}
%\morteza{Added the remark to address this point.}

%\fei{You can say most of this in the definitions section and by defining a $\delta_{i,j}$ function to capture the changes.  I would just define a function that allows you to return the number of nodes $|u.type|$ that exist in each fragment. } \morteza{I guess it is better to count the number of edges as $|nodes|$ will not give us a good estimation.}

%\newtext{\stitle{Communication cost.} For a given partitioned temporal graph $\{\mathcal{P}_1, \dots, \mathcal{P}_n\}$ \cyan{Fragments $\mathcal{F}$?} and a \tgfd $\sigma \in \Sigma$, we compute the communication cost $C_i(\sigma)$ as the total number of edges that needed to be shipped to machine $M_i$. To this end, for each temporal partition $P_j$ ($j\neq i$) and each snapshot partition \cyan{What is the difference between temporal partition and "snapshot partition"?} $G_k^j$ ($k=1,\dots, T$), we count the number of edges $e(u,v) \in G_k^j$, such that either $L_k(u)$ or $L_k(v)$ is equal to a type in pattern $Q$ of $\sigma$.}  \cyan{Be careful with your notation and super, sub-scripts being different across definitions.  Before it was $G$ superscript "r" and superscript "j".  I did not understand the intuition of the last sentence what it's computing and why.}

\subsection{Initial Workload Assignment}\label{sec:WorkloadAssignment}

We seek an assignment of joblets to the worker machines such that \ccost, and the makespan minimized. To this end, we use the technique of~\cite{shmoys1993approximation} to define a combined objective function to minimize both \ccost and makespan, where there exists a 2-\emph{approximation} algorithm. In this algorithm, we need to perform a bisection search on the range of possible makespan values. To this end, we maintain all the assignments that have objective function value less than half of the objective function value of the best current assignment that minimizes the makespan. At the end, among all maintained assignments, we select the one with minimum makespan. We need to solve the linear program of the general assignment problem at most $log(kP)$ times, where $k$ is the total number of joblets and $P$ is the maximum workload among all joblets~\cite{shmoys1993approximation}.


\subsection{Adaptive Load Balancing}\label{sec:AdaptiveLoadBalancing}

Initial workload assignment is done based on the first snapshot $G_1$ and then $M_c$ sends updates to the corresponding machines based on the assignment.  However, there might be cases that one machine becomes overloaded as the changes are coming. In this section, we try to detect burstiness in the workloads and then resolve data skewness by re-balancing the overloaded machines.

\subsubsection{Handling Burstiness}

Burstiness happens when one fragment $F_{ij}$ is assigned subgraphs that \newtext{change} substantially compare to other subgraphs in other fragments. For example, in a social network, one person might become a celebrity after some points in time and the subgraph around that person \newtext{changes exponentially compare to other subgraphs}. In this case, our initial workload assignment is imbalanced and we need to re-balance it. To this end, we first need to detect burstiness before starting the new snapshot and then re-balance the workload if needed. Note that the re-balancing is time consuming and it might involve data shipments as we might assign joblets to new machines. \eat{Since the matching time exponentially grows by the size of the subgraph, we trade-off the overhead of workload re-balancing by detecting large subgraphs and overloaded workers.}
The coordinator $M_c$ maintains the size of each subgraph in terms of the number of edges. This can be initially computed when $M_c$ defines the workloads. Before sending the updates to the workers, $M_c$ computes the size of each subgraph based on the newly added or removed edges. Following the incremental algorithm of Section~\ref{sec:incdetect}, we need to perform two subgraph isomorphism for each single change. We compute the workload of each change using the Equation~\ref{eq:unitworkload} and aggregate it for all the changes for each joblet. $M_c$ computes the workload on each Machine $M_i$ by aggregating the workloads of the joblets assigned to $M_i$. Makespan of the new snapshot would be the largest workload among all machines, call it $\mathcal{J}_{makespan}$. $M_c$ estimates the optimal makespan by $\mathcal{J}_{optimal}=\dfrac{\sum_{j=1}^{n}\mathcal{J}_{ij}}{n}$. If $\mathcal{J}_{makespan} \not\in [\mathcal{J}_{optimal},2\times\mathcal{J}_{optimal}]$, then it means we have violated the 2-\emph{approximation} guarantee of the initial joblet assignment and need to re-balance the workload by re-assigning the joblets.

\subsubsection{Workload Re-balancing}

After the burstiness is detected, $M_c$ calls a re-balancing procedure to make sure that no machine is overloaded. To this end, we use the 2-approximation technique of~\cite{aggarwal2003load}. We estimate the communication cost of the joblets (Equation~\ref{eq:datashipment}) as the cost of relocating. After re-balancing the workload to minimize the makespan, $M_c$ sends the joblets to their new machines along with a list of edges to be shipped to other machines (if there are any). It also updates its own list on where a subgraph $G(v,d)$ resides for each candidate node $v$. Then, $M_c$ starts the new round by sending the updates of the new timestamp to the corresponding machines.


%%%%%%%%%%%%%%%%%%%%%%%
\eat{

We define a general assignment problem as follows: for each joblet $\mathcal{J}_p$ (1) we estimate the size of the joblet $|\mathcal{J}_p|$;
\eat{I think by the defn. of joblet is understood to be the amount of work, so no need to define it as size.}\eat{In the definition, we define a joblet with a subgraph. However, the size of the joblet is based on Equation 2. The size of a joblet gives us a perspective of an estimated amount of time we need to find the matches around the subgraph. The size exponentially grows as the number of edges increases.}
(2) for each machine $M_j$ ($j=1, \dots, n$), estimate the communication cost of assigning $\mathcal{J}_p$ to $M_j$ as $CCost_{pj}$. The general assignment problem is to solve the following linear program to find the values of the assignment array $X$:  
\begin{equation} \label{eq:generalassignment}
\begin{split}
    minimize: \sum_{p=1}^{m}\sum_{j=1}^{n} CCost_{pj}\times X_{pj}\\
    minimize: \sum_{p=1}^{m}\sum_{j=1}^{n} |\mathcal{J}_p|\times X_{pj}\\
    such \ that: \sum_{j=1}^{n} X_{kj}=1 \ \ for \ p=1, \dots, m\\
    X_{pj}\geq 0 \ \ for \ p=1, \dots, m \ \ \;for \ j=1, \dots, n
\end{split}
\end{equation}
To solve this linear program, we use an extension of makespan minimization~\cite{shmoys1993approximation} to find an assignment of $W_{\Sigma}$ to $n$ machines.
}

\eat{\fei{[Aug 11th update] Morteza: this needs revision based on our discussion that using the lower/upper bounds outlined in the Corollary of the GA paper, we check if the changes go beyond the upper/lower bounds then we must re-assign to maintain the guarantees.}

\fei{(1) So the approximation is not guaranteed.  There needs to be discussion about this otherwise there will be criticism about how we manage the cost and time to prevent them from becoming unbounded.}

\fei{(2) There is not much in this section other than defining notation, and saying we use [31] to minimize the makespan. This section needs to be elaborated to discuss how we adapt the workload assignment in light of incoming changes.  E.g., if changes allow us to still bound the costs and runtimes per joblet to machine within a lower to upper bound, can we still provide some guarantees.  If so, how can we do this?}
}
%\fei{To make the connection more clear between total workload, workload per machine and joblets, one way is to define $W_j(.)$ which are composed of joblets and now you are trying to define $W_j$ across the machines.  Comm cost is defined per machine as the messages needed to be sent per machine.  This simplifies the discussion to computing workload per machine.} \morteza{I have defined workload based on joblet, machine and $\Sigma$ and revised the above text accordingly. However, since we have a fine grained workload assignment, our items to be assigned are joblet and the communication cost has to be considered in the general assignment problem based on joblets, not machines. }

%\fei{[DISCUSSION POINT] This is a good high-level overview.  However, it will need to be expanded with more details of how the assignment is done and the intuition of this solution, and the approximation.  We have at least two cases in our problem setting.  I recall Yinghui mentioning that for the \emph{static} case where the cost and weights do not change, the 2-approx. holds.  This is one case for us.  However, there is a dynamic case where $\delta$ changes impact the comm. cost after $t_1$, and the assignment problem approximation no longer holds.  I recall Yinghui making a note of this, and we should outline this in the paper as well.  I leave this here for reference as a point of discussion.}

%%%%%%%%%%%%%%\input{Algorithms/parallelTED}

\subsection{Parallelized Matching and Error Detection}

%\fei{Matching can be done on each worker machine based on local data.  How are pairwise matches compared and errors detected if matches are on separate machines? We ship some of these matches to a single worker node (as considered in the previous estimation and assignment step), and then aggregate errors via UNION  at the coordinator?}
In this section, we explain how parallel \tgfd error detection (\tedparallel) works. Given a set of \tgfds $\Sigma$, a fragmented temporal graph \tempgraph, a coordinator $M_c$ and a set of workers $\{M_1,\dots,M_n\}$, the task is to find the set of violations \errorSigma \ in parallel. Assuming $M_c$ has full view over \tempgraph, we first define the set of all joblets \totalworkload and then estimate the communication cost of assigning each joblet to the workers. We then find \jobletSigma as the set of workloads for each machine $M_j$ by solving the general assignment problem of the Section~\ref{sec:WorkloadAssignment}. We send each \jobletSigma to the corresponding machine along with a list of edges to be shipped to other machines. Recall that this list can be computed using the communication cost function in Section~\ref{sec:workloadAndEstimation}. 

At a timestamp $i$ (initially 1 for the first timestamp), each machine $M_j$, receives a set of joblets \jobletSigma. After shipping all necessary data to other machines and receiving the data from others, $M_j$ merges the received data with its own fragment $F_{ij}$. Then, for each joblet $\mathcal{J}(\sigma,F_{ij}, \mathcal{G}(v',d)) \in$\jobletSigma, it finds/maintains the matches incrementally using our \tedincremental algorithm of Section~\ref{sec:incdetect}. For each match $h_{t_i}(\bar{x})$ of $\sigma$,  $M_j$ generates a message in the form of \emph{<key,value>} as <$(\sigma),(h_{t_i}(\bar{x}),flag)$>. We use a bit to distinguish between matches that are appeared or removed in the incremental update using \emph{flag}. After sending the matches, $M_j$ waits to receive the new snapshot to start the next round and compute the matches at the next timestamp. If the re-balancing procedure was triggered at the $M_c$, then each machine $M_j$ might receive a set of joblets to be shipped to other machines (resp. receive from other machines) before starting the next timestamp.

The coordinator receives the messages from all machines and order the messages based on their keys.  
More specifically, for each $\sigma \in \Sigma$ and a timestamp $t_i$, it receives the messages as <$(\sigma),List\{(h_{t_i}^1(\bar{x}),flag), \dots , (h_{t_i}^s(\bar{x}),flag)\}$> assuming there exist $s$ matches of $\sigma$ across all machines.  Recall the \tedincremental algorithm of Section~\ref{sec:incdetect}, $M_c$ creates and maintains $\Pi_X$ for $\sigma$ and runs the error detection when the matches of the new timestamps come. After receiving the matches from all workers for all timestamps, $M_c$ compute the set of violations \errorSigma.  

%\fei{is this the same $k$ used for joblets?} \morteza{Changed to $s$.}\fei{ Don't really understand the purpose of the add/remove here.}\morteza{Changed to \emph{flag}. The coordinator needs to know if a match is just appeared at timestamp $i$ or it is disappeared because of a change at timestamp $i$. The coordinator maintains the intervals to detect violations.} \fei{ Why can't we just reference the inc matching algorithm used in sequential version?}\morteza{I trimmed the previous paragraph and referenced to Section~\ref{sec:incdetect} to find the matches. However, the matches have to be sent to the coordinator for pairwise comparison, because the machines do not have the global view.} \fei{What are you doing here that is different than sequential w.r.t. error matching?  How are pairwise comparisons done across nodes?} \morteza{I am finding the matches in parallel, then send the matches to the coordinator and the coordinator finds the violation by pairwise comparisons.}

%%%%%%%%%%%%%%\newtext{\stitle{Algorithm.} For a given set of fragments \temporalfragmentset{n} and a set of \tgfds $\Sigma$, algorithm \tedparallel finds the set of violations \errorSigma.
%\fei{Workers/machines and coordinator can be defined in the earlier section.}  
%\fei{It looks like you don't need the defn. of fragment based on time because the current model is not considering subsequent changes to a fragment at time $t$, so there is no need to access a fragment at a specific time.  We should discuss to clarify.} 
%%%%%%%%%%%%%%The algorithm works as follow: (1) For each $\sigma \in \Sigma$, it first defines the corresponding joblet \jobletsigma and estimates the workload of each joblet $W(J)$. 
%\cyan{I would suggest having a section that just introduces all your concepts and notation first to separate definitions from algorithm explanation.  How is this induced graph computed and how is it related to communication cost, which is defined over a snapshot?  The connection between joblet and communication cost needs more details please.}
%%%%%%%%%%%%%%(2) For each joblet, it estimates the communication cost of assigning the joblet \jobletsigma to machine $M_i$ ($i=1,\dots, n$).
%\fei{So a joblet $J$ is the work unit, and how is this defined?  If you are measuring the amount of work of a joblet would take on a machine, it would be good to incorporate the fragment $F_j$ on machine $j$ (in Workload estimation), and sum across the machines.  The fragment is not used in any of the estimations.} \morteza{Joblets and the workload of joblets are computed in the coordinator. We assume coordinator has full view to the \tempgraph.} 
%\fei{Is there a workload allocated per machine/fragment?  Something like $J(\sigma, F_j)$ or $W_j(\sigma, G)$ (as in the GFD paper) for $j = [1,n]$.}
%\fei{The defn of joblet and workload estimation has to be revised based on the June 2 discussion.}
%%%%%%%%%%%%%%(3) Reducing to general assignment problem~\cite{shmoys1993approximation} (to be explained shortly), we find a \emph{2-approximation} solution to assign joblets to machines in order to minimize the total communication cost and total run time (\emph{makespan}). 
%\cyan{This needs more detail of what the assignment problem is, how your pieces correspond to the assignment problem, and how the assignment problem is solved. More details needed here.}  
%%%%%%%%%%%%%%(4) After joblets are assigned, each machine $M_i$ ships relevant data from fragment $\mathcal{F}_i$ to other machines. It also receives data from others and merge with its local fragment $\mathcal{F}_i$. (5) Using \tedincremental algorithm, each $M_i$ finds the violations of the assigned joblets locally and sends \errorsigma to $M_c$. (6) Finally, the coordinator $M_c$ computes \errorSigma = $\bigcup_{\sigma \in \Sigma}\mathcal{E}($\tempgraphsigma$, \sigma)$.
%\cyan{Can we include the overview the Yinghui suggested with three main steps: computing matches, pairwise comparisons and error detection.  Describe how each of these steps is done and feeds into the next step.} 
%%%%%%%%%%%%%%Algorithm~\ref{alg:tedparallel} provides \tedparallel details.}




%\fei{(1) So this sounds like a new workload assignment after each timestamp, is this what you mean?  How do we justify the overhead? (2) Data skewness and burstiness refer to different aspects: (a) burstiness when updates (over a short period of time) cause a subgraph to change dramatically (centrality, node degree, etc); (b) smaller number of changes that occur over a longer period of time over a fixed set of subgraphs that lead to a large number of matches (data locality among these subgraphs is high). }

%\fei{This sounds quite vague.  How is $W_{min}$ computed?}\morteza{Removed $W_{min}$ and cited the relevant paper. The details of the re-balancing algorithm is a lot and I just cited the paper as what they did in the GFD paper.} \fei{ We discussed with Yinghui about re-distributing only the incoming changes to avoid large comm. cost.} \morteza{We need to re-distribute the \emph{joblets} not just the changes. Each joblet contains the subgraph and if we want to re-assign the joblet, we need to re-locate the subgraph. The cost of re-locating (as communication cost) is part of the re-balancing problem and the cited paper tries to minimize it based on a either a budget or maximum number of re-locating.}

%%%%%%%%%%%%%%%%%%%%%%%%%%% For reference
%\begin{enumerate}
%    \item Define model: Graph fragmentation, joblets, worklets
%    \item Workload estimation model/formula
%    \item Assignment problem
%\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Runtime complexity.} 

We show that error detection using \tedparallel is feasible by proving that it is \emph{parallel scalable}\cite{kruskal1990complexity}. First, lets discuss the complexity of $\tedincremental$ algorithm as we run it in parallel on $n$ machines. Let $T_{inc}(|\Sigma|,|$\tempgraph$|)$ be the time to compute \errorSigma \ using \tedincremental algorithm in one machine. To compute $T_{inc}$, let $G(d,\hat{v})$ of a candidate node $\hat{v}$ be the largest $d$-hop subgraph among all candidate nodes across all fragments. It takes $O(|G(d,\hat{v})|^d,\Sigma)$ to compute matches $\mathcal{M}$ in the first timestamp. For the subsequent timestamps, the complexity is bounded by the number of changes $|\delta_{i,j}|$ and it takes at most $O(|\mathcal{M}|\times |G(d,\hat{v})|^d \times |\delta_{i,j}|)$. Based on this, $T_{inc}=O(|G(d,\hat{v})|^d,\Sigma) + O(|\mathcal{M}|\times |G(d,\hat{v})|^d \times |\delta_{i,j}|)$. 

\tedparallel algorithm is \emph{parallel scalable} if it takes at most $O(T_{inc}/n)$ time, where $n$ is the number of machines. Given the total workload \totalworkload, we observe that: $T_{par} = \dfrac{O(T_{inc})*c_1}{n} + (n \times |\Sigma| \times|$\totalworkload$|)^{c_2}$, where $c_1$ and $c_2$ are constants and the second part is the time complexity of the assignment problem and re-balancing procedure. $T_{par}$ is \emph{parallel scalable} since $\dfrac{O(T_{inc})*c_1}{n} > (n \times |\Sigma| \times|$\totalworkload$|)^{c_2}$, while $n\leq|$\tempgraph$|$.

==> parallel_orig.tex <==
\section{Parallel Error Detection}
\label{sec:parallel}
%\fei{Morteza: is there a revised version of this I can read before the May 26th meeting?  We discussed several changes in our last meeting, and looking for the revisions here, and the new content as per the May 21st items in the document (the purple highlights).  As mentioned in the last meeting, please email me with what to read (FYI, I have 10:30-12pm tomorrow to read). }

%fei: why is temporal and spatial locality dependent on parallel execution?  Could this not be exploited in the sequential case?  If there is some argument I'm missing that ties locality to parallelism, then you can extend for your thesis.  
\eat{
For an increasing number of \tgfds, there will be increasing similarity in data accesses among the graph pattern queries.  Past work have shown that queries over social network graphs share over 82\% spatial similarity~\cite{graphm}.  In addition, the same subgraphs may be accessed by different queries over the same time interval.  To reduce this data access overhead among graph pattern queries, we exploit this spatial and temporal locality, and propose a parallel algorithm.  
}
%\subsection{Overview}
The error detection problem is tied to validation where we want to compute \errorSigma,  the set of violations of $\Sigma$ in \tempgraph. Error detection for \tgfds incur additional challenges.  Instead of retrieving matches at a single point in time, matches may occur at any  \snapshot \ for $t \in [1, T]$, and are compared pairwise $(h_{t_i}(\bar{x}),h_{t_j}(\bar{x}))$, where $|t_j - t_i| \in \Delta$, to check dependency conditions $X \rightarrow Y$.  (Without loss of generality, we assume attribute $Y$ contains a single literal $y$).  For each \snapshot, we must compute all matches of $Q$ that are isomorphic to a subgraph of \snapshot.  A naive, batch approach finds all matches for \snapshot, and then re-computes all matches for subsequent $G_{t+1}$ from scratch, for all $\sigma \in \Sigma$.   The complexity of subgraph isomorphism is known to be \npc \ for general graphs~\cite{GJ90}, making the batch approach infeasible for large graphs, and motivating the need for incremental and parallel solutions.   

Large, evolving graphs pose additional efficiency challenges over static graphs, where delta changes between snapshots need to be incorporated.  It has been shown that most graph changes affect a small portion of the graph, involving a similar set of entities.  For example, recent studies have found only 5-10\% of nodes are updated weekly~\cite{FJJ11}, and 80-99\% of the changes are highly localized~\cite{BBT18}.  In our empirical study using DBPedia, we found 82\% of updates and insertions are localized to a small set of entities.  Given this, we first take an incremental approach towards \tgfd error detection.  We avoid recomputing matches from scratch each time a change occurs, and avoid the exhaustive comparison among all matched pairs.  We build upon past work by Fan et. al. that proposes \isounit, an incremental matching for subgraph isomorphism algorithm~\cite{FJJ11}.  

that updates a set of matches by localizing the subgraph isomorphism operation to the induced subgraph of \snapshot \ containing only nodes within a given distance from the updated nodes~\cite{FJJ11}.  

We build upon the incremental matching for subgraph isomorphism algorithm, \isounit, proposed by Fan et. al.,~\cite{FJJ11}, where we incrementally check for new violations due to changes in \snapshot. 

%****************
To realize \tgfd error detection for large-scale graphs, parallel algorithms are needed.  We propose \tedparallel, a \emph{\uline{Parallel} \uline{T}GFD \uline{E}rror \uline{D}etection} algorithm that balances finding matches and \tgfd validation across a set of (machine) workers, and  minimizes the communication overhead.  To adapt to incoming changes, particularly localized updates that create bottlenecks and increase latency, we propose a workload re-balancing strategy among the workers.  We design \tedparallel over fragmented graphs to consider settings when graph replication at each node is too expensive.  We introduce our workload model next.


%fei{You can use and revise for your thesis..}
\eat{
Real world temporal graphs are large and we need extensive computational power to find the violations of \tgfds if we process the graph in one machine. We consider a cluster of machines to detect the violations in parallel including a coordinator $M_c$ and a set of $n$ workers $M_1,\dots, M_n$. Assume a graph fragmentation exists and we assign each fragment to a machine in the cluster. 
Each machine is also assigned a set of joblets as unit workload to find the matches in its fragment locally. However, since the graph is fragmented, there might be nodes/edges in other fragments that need to be shipped to a machine to find the violations. Therefore, $M_c$ identifies parts of the fragments on each machine that needs to be sent to other machines.
%each machine needs to collect parts of its fragment that are needed in other machines and send over the data.  
We compute the amount of data shipment as a factor, namely \emph{communication cost}, in the process of assigning \tgfds to each machine. As another factor, for each \tgfd $\sigma \in \Sigma$, we estimate the number of matches of $\sigma$ and then estimate the amount of work needed to find all the matches.
%\fei{Don't really understand the point of this last sentence, we need to find matches regardless.  What is a "light process"?} 
Based on this, the problem of Parallel \tgfd Error Detection (\tedparallel) consists of the following steps:
\begin{itemize}
    \item Define the workload as set of joblets. ($M_c$)
    % based on the potential matches of each \tgfd in $\Sigma$
    \item Assign workloads the workers such that the communication cost and makespan is minimized. ($M_c$)  
%    \fei{I assume runtime means a "balanced" workload? If so, you should make this explicit.}
    \item Ship the necessary data (nodes and edges) to other workers and receive data from them, based on the assigned workloads. (workers)
    \item Find the matches of the assigned joblets and send the matches to $M_c$. (workers) 
    \item \newtext{Receive, maintain and compare the matches from the workers to find any violations.} ($M_c$) 
    %After the workers are done finding the matches, the coordinator receives and maintains the matches from workers. When the matches are received, it finds the violations for the matches so far. ($M_c$) 
    \fei{$M_c$ needs to compare matches from different machines right and handle matches that may be violated (with past matches from other machines) as changes arrive.}
    \item Check if the next timestamp makes the workload imbalanced. Re-balance the workloads if necessary. Send the next timestamp to the workers. ($M_c$)
%    \fei{What does it mean send new timestamp?  Isn't it a re-assignment of \tfds to workers?}
    \item repeat the last four steps until no changes remain. ($M_c$ and workers)
    %\morteza{I have shortened the bullets as per your first comment on Section 6.4}
    %%%%\item Find the violations based on the received matches. ($M_c$)  \fei{Is the matching not done incrementally?  You only do it at the end?}
    %\item \fei{[DISCUSSION POINT] How are incremental changes considered?  For example, a new edge appears at time $t_3$?  If changes are sent to all machines, then this needs some discussion.  Could a new match could occur on machine $M_2$ at $t_3$ (edge insertion) for $\sigma_1$ on machine $M_1$?} %\morteza{added a new bullet point}  \fei{Which bullet point?}
%    \item \fei{(1) Just to clarify: $M_c$ estimates the total workload and this consists of joblets that are defined w.r.t. the subgraphs that exist on each machine.  After this has been estimated across all fragments (machine/workers), then the assignment is done to minimize communication cost and balanced workload. (2) this is the "adaptive" part that can trigger a re-balancing right?} \morteza{(1)Yes. exactly. (2) I have added the adaptive re-balancing.}
\end{itemize}
}


%Given a temporal graph \tempgraph \ and set of \tgfds $\Sigma$, the parallel algorithm is to compute \errorSigma \ such that: (1) the communication cost (data shipment) is minimized and (2) total run time (\emph{makespan}) is minimized.}

%For reference.
%\begin{enumerate}
%    \item discuss idea of how this is going work
%    \item main components: matching, pairwise comparison and error detection
%    \item Parallel scalable, complexity
%\end{enumerate}
%%%%%%%%%%%%%%%%

\subsection{Workload Model}
\label{sec:workload}

%Before explaining the description of the \tedparallel algorithm, we provide some definitions.


Consider a set of $n$ worker machines $M_1 \ldots M_n$, and a coordinator machine $M_c$.  A fragmentation of \tempgraph \ across the machines is a set of fragments \fragments, each a subgraph of snapshot $G_i$ on machine $j$, where $i \in [1, T], j \in [1, n]$.
Given $\Sigma$ and a fragmentation \fragments, we compute \errorSigma \ in parallel such that the workload assignment across the $n$ machines is distributed as evenly as possible, and the communication cost between the machines is minimized.  

It is important to accurately estimate the number of matches for query pattern $Q$ for each $\sigma \in \Sigma$.   We estimate the cardinality of $Q$ against fragments \fragments \ by decomposing $Q$ into query pattern paths \querypath \ with variable and value constraints, where $k$ ranges from 1 to the number of query paths in $Q$, which are then aggregated to find the result set of $Q$. \eat{We compute the expected workload by estimating the number of subgraph matches for each $\sigma \in \Sigma$.}  Since a given fragmentation may split a match of \querypath \ w.r.t. $\sigma$ across two or more machines, we estimate the data that must be copied between machines to compute a match, as the communication cost.  Each machine $M_j$ locally computes the matches against $F_{ij}$, and performs local validation w.r.t. $\sigma$ to compute \errorsigmaj, and then sends the matches and errors to $M_c$.  \eat{Changes to \fragment \ are sent to $M_j$, which may add or remove  inconsistencies from \errorsigmaj \ and \errorsigma.  We handle this by  \tbf} Changes to \fragment \ (edge insertions/deletions, attribute updates) can lead to workload imbalance across the machines where some machines incur an increasing burden of the workload.  If runtimes at any machine lie beyond the given lower and upper bounds, then we re-balance the workload via a new workload assignment. 


\subsubsection{Path Queries, Joblets and Jobs}

%fei: you can re-use for your thesis if you'd like.  I have simplified above, we already stated in Sec.2 what type of changes. 
\eat{
\begin{definition}
Given two snapshots $G_i$ and $G_j$, $\delta_{i,j}(G_i,G_j)$ contains all the differences between $G_i$ and $G_j$ including: edge insertion and deletion, node attribute insertion and deletion.
\end{definition}
}
%\begin{definition}
%Given a snapshot \snapshot \ and a natural number $n$, \snapshotfragmentset{t}{n} is a set of $n$ %disjoint snapshot fragments such that $\bigcup_{i=1}^{n} G_t^i = G_t$. 
%\end{definition}

%\fei{What does $n$ represent?  If number of machines, you are partitioning a snapshot graph over $n$ machines?  Can we not say "Let $G_{i}^j$ represent the subgraph of $G_i$ on machine $j$?  We call each of these subgraphs a fragment.}

%fei: same comment as before: use for your thesis if you'd like and simplified.
\eat{
\begin{definition}
Let $G_{i}^j$ represent the subgraph of $G_i$ on machine $j$. 
\newtext{Let $\{F_{i1},\dots,F_{in}\}$ be a set of \emph{fragments} of \tempgraph \ at timestamp $i$, 
where each fragment $F_{ij}$ = \{$G_1^j$, \snapshotdiff{1}{2}{G_1^j,G_2^j}, \dots, \snapshotdiff{(i-1)}{(i)}{G_{i-1}^j,G_{i}^j}\}. A fragment $F_{ij}$ is located at machine $j$}.

%\fei{Notation is getting messy, let's discuss to cleanup, e.g., $F_{ij}$}
%%%%%%%%%%%%%%%%%Let $\{G_1^1,\dots, G_1^n\}$ be a set of fragments of $G_1$ on $n$ machines.
%*** I removed this for now ***
%We call each of these subgraphs a \emph{snapshot fragment}
%\fei{What is the significance of the word "snapshot"?}.\morteza{I want to make a difference between $G_i^j$ and $\mathcal{F}_i$. I want to call the latter one \emph{fragment} as you suggested, so have to call the former something else. Do you have any other suggestion?} \morteza{We need to refer to $G_1^j$ later to compute the communication cost.}
%Let \temporalfragment{i}$^t$ denotes the fragment at time $t$, where we apply the changes \snapshotdiff{1}{2}{G_1^i,G_2^i}, \dots, \snapshotdiff{1}{2}{G_{t-1}^i,G_t^i} in a sequence on the first snapshot fragment $G_{1}^i$
\end{definition}
}
%\fei{Does it matter to reference the snapshot $G_1$?  If not, I'd suggest cleaning up the notation and using $F_j$ to represent the fragment on machine $M_j$.  This allows follows more standard notation used in past papers.} \morteza{Revised to make it consistent.}

%\fei{Be careful to not overload your use of index $i$, it should be used to represent one series.    The $\delta$ function was defined with $G_i, G_j$ with no superscripts.  I would recommend you stick with one definition of fragment, just define it once.}\morteza{Revised to consistently use $j$ to refer to machines}

%\fei{How about something like: "Let $F_{i}^j$ represent the \emph{fragment} of snapshot graph $G_i$ located on machine $j$, $j = \{1 \ldots n\}$.  We assume a partitioning of $G_i$ into fragments across $n$ machines, such that each fragment $F_{i}^j$ is the subgraph of $G_i$ on machine $j$. Intuitively, we partition snapshot $G_1$ and all subsequent changes $\delta_{i,j}$ between two snapshots $G_i, G_j$ are applied to the corresponding fragment.}

% \begin{definition}
% Given a temporal graph \tempgraph, a node $u$ and a distance $d$, $Candid(\mathcal{G}_T, u, d)$ is a \emph{list} of candidate matches of $u$ in \tempgraph. A node $v$ exists in $Candid(\mathcal{G}_T, u, d)$, if (1) $v$ has the same type as $u$ in the first snapshot $G_1$ (\emph{i.e.,} $L_1(v)=L(u)$) or (2) for a snapshot difference \snapshotdiff{t_1}{t_2}{G} that $L_{t_2}(v)=L(u)$, there exists a change within $d$ hops of $v$.
% \end{definition}

\eat{
\begin{definition}
Consider a \tgfd $\sigma=(Q[\bar{x}],\Delta, X \rightarrow Y)$ and $\hat{c}$ as a center node with minimum radius in $Q$, where \emph{radius} is the longest shortest path between $\hat{c}$ and other nodes in $Q$. We define $Candid(\sigma,F_{ij})=\{v_1,\dots, v_k\}$ as a set of candidate nodes in $F_{ij}$ that are from the same type of $\hat{c}$ \emph{i.e.,} $L(\hat{c})=L(v)$ for all $v\in Candid(\sigma,F_{ij})$.
\end{definition}  
\fei{The chosen center node's type is used to define the subgraph $G$ in the joblet.  So in Fig 1, if you pick node $y$ (position) in $Q_2$, then we define Candid($\sigma$, $F$) and $G$ in joblet, to include nodes based on type position and nodes a distance $d$ from this node.    Given this, I think in Defn. 6.1, you mean the radius to be the longest (shortest) path to \emph{any} node in $Q$ so that you can get coverage for all nodes in $Q$.  Remove "and other nodes in Q" is ambiguous and I interpret to mean ALL other nodes.}
\todo[inline]{Morteza: if you meant "any" then please remove this block from Defn. 6.1 and my red comment.}
}
%\fei{If Candid() is dependent on $F_j$, then I suggest you include it as an input in addition to $\sigma$. }

%\fei{minimum diameter to what?  Between c and what? \morteza{Revised.} I assume this is updated as $\delta$ changes come in?  }

For each $\sigma \in \Sigma$, we decompose the query pattern $Q$ into a set of path queries $Q_k$, where each $Q_k$ is a maximal path from vertices $v_1$ to $v_m$ in $Q$, as a sequence $(v_1,a_1,v_2), \ldots , (v_{m-1}, a_{m-1}, v_m)$ for some $k, m \geq 0$.  Each $(v_l,a_l,v_{l+1})$, $l < m$, is an edge in $Q$.  We augment  $Q_k$ with value constraints defined by the literals $x \in \bar{x}$, i.e., $v_{l}.A$ is in $X$ or $Y$, for an attribute $A$.   We apply cardinality estimation techniques from query optimization over ontological queries to estimate the matches for each $Q_k$~\cite{SRK07}.  For a query pattern $Q$, the result set (matches) w.r.t. a literal $x$ is computed as the intersection of the result set for each query path $Q_k$ containing $x$.  The cardinality of this result set is upper bounded by the smallest result among the $Q_k$ path queries.   We compute the result set of $Q$ as the union of the result sets over all literals $x \in \bar{x}$, and the cardinality is computed as the sum of these results aggregated over all literals~\cite{SRK07}. 

Let $v_{k}$ be a center node with minimum radius in $Q_k$, where the radius is the longest, shortest path between $v_{k}$ and any node in $Q_k$.  We define $Candid(Q_k,F_{ij})$ as a set of candidate nodes in \fragment \ of the same type as $v_k$, and satisfy the attribute literals defined in $v_{k}$.   For example, Figure~\ref{fig:matchingExample}(a) shows two (maximal) query paths $Q_1'$ and $Q_2'$ of the pattern $Q_3$ in Figure~\ref{fig:mainExample} with the literal set $\{z=$\lit{McMaster}$\}$.



%Let $\bar{v_{k}}$ denote the set of center nodes for a pattern $Q$ of $\sigma$.
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figures/matching.png}
    \vspace{-0.3cm}
    \caption{Query paths with matching.}
    \label{fig:matchingExample}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
 
\eat{
\begin{example}\label{example:QueryPath}
%\fei{Add a visual figure here so it's clear for the reader, showing $Q$, the corresponding $Q_k$ query paths, sample edge $(v_1,a_1,v_2)$, $v_k$ for a $Q_k$, and $\bar{v_k}$.}
Figure~\ref{fig:matchingExample}(a) shows two (maximal) query paths $Q_1'$ and $Q_2'$ of the pattern $Q_3$ in Figure~\ref{fig:mainExample}. Both $Q_1'$ and $Q_2'$ include node and edge labels, and the literal set \eat{are maximal query paths that there exists no query path that is a subset of them and the union of $Q_1'$ and $Q_2'$ equals to $Q_3$. Moreover, each query path can be considered as a sequence of edges, \emph{e.g.,} $($\lit{advisor}, \lit{supervise}, \lit{student}$)$ and $($\lit{student}, \lit{study}, \lit{university}$)$ for $Q_1'$, where the university has the literal set} $\{z=`$\lit{McMaster}'$\}$.
\end{example}
}
\eat{
\begin{definition} (\emph{joblet}) 
\newtext{A joblet  is defined based on the nodes in $Candid(\sigma,F_{ij})$ for each fragment $F_{ij}$ and each \tgfd $\sigma \in \Sigma$. A joblet represents a \emph{work unit} in our distributed setting. More specifically, for a given \tgfd  $\sigma=(Q[\bar{x}],\Delta, X \rightarrow Y)$ and a fragment $F_{ij}$, $\mathcal{J}=(\sigma,v,F_{ij},G(v,d))$, where (a) $\sigma$ is the corresponding \tgfd; (b) $v$ is a candidate node in $Candid(\sigma,F_{ij})$; (c) $F_{ij}$ is the fragment that contains $v$; and (d) $G(v,d)$ is the induced subgraph $d$-hops around node $v$, where $d$ is the diameter of $Q$. 
Let $W_{ij}(\Sigma,$ \tempgraph) be all the joblets aggregated for $F_{ij}$ and $W(\Sigma,$ \tempgraph) be the aggregation across all $j$. 
%\fei{After reading this, the sub and superscript can be replaced with $F_{ij}$ and referred to as $F_i$ when needed, and the former with timestamp when needed. } 
Since we have a fixed set of nodes in \tempgraph, the total number of joblets is fixed and is independent of the timestamps.}
\end{definition}
%\todo[inline]{See my questions on slack regarding Defn 6.1.  If Defn. 6.2 is OK, please remove Defn. 6.1, otherwise, let me know inconsistencies.}
}

%JOBLET Defns.
\begin{definition} (\emph{joblet}):
Let \joblet \ represent a \emph{joblet} denoting a unit of work to compute matches of $Q_k$ on fragment $F_{ij}$ over \tempgraphk = $\{G_1(v',d), G_2(v',d), \ldots , G_{i}(v',d)\}$, $v' \in $ \candQk \ such that $\forall s, s' \leq i, |s' - s| \in \Delta$.  The fragment \fragment \ contains node $v'$, and \tempgraphk \ are the induced subgraphs $G_t(v',d)$ $d$-hops around $v'$ for diameter $d$ of $Q_k$ for $t \leq i$. 
\end{definition}

Intuitively, \tempgraphk \ are the induced subgraphs from \tempgraph \ that must be checked to compute the matches to $Q_k$.  
%\fei{revise induced temporal subgraphs, and $Q_k$ vs. $\sigma$ in joblet defn, and below defn.}

\begin{definition} (\emph{job}): 
Let \job \ be a \emph{job} representing the workload to validate a \tgfd $\sigma$ with pattern $Q$.  A job consists of the set of joblets for all path queries $Q_k$ corresponding to $Q$ where $v' \in $ \candQk \ of \tempgraph \ in $F_{ij}$.  \eat{containing node $v \in Candid(Q_k,F_{ij})$.  $G(v,d)$ is the induced subgraph $d$-hops around $v$ for diameter $d$ of $Q$. }
Let \jobSigma \ represent jobs for a set of \tgfds $\Sigma$,  i.e., $\cup_{\sigma \in \Sigma}$ \job.
%$\sigma \in \Sigma$ for a given $F_{ij}$. 
%and \jobletall \  denote all joblets across all snapshot graphs and machines.  
\end{definition}

%\noindent \textbf{Overview.}  
We estimate the workload to compute query matches by estimating the size of joblets, jobs and the expected communication cost between machines.  Given these estimates, we derive an initial assignment of jobs to machines that balances the workload across the machines.  To compute \errorSigma, we compute the matches of $Q$ for all $\sigma \in \Sigma$.  Lastly, we adjust our job estimations and workload assignments to adapt to changes in \tempgraph.

%\fei{Morteza: Need to give an overview of the main steps of this parallel error detection: (1) initial assignment via joblet size estimation; (2) communication cost estimation; (3) (initial) general assignment; and (4) query matching and error detection; (5) re-estimation of matches due to changes; (6) workload re-balancing.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Workload Estimation}
\label{sec:estimation}

We describe our estimations, and define an assignment of jobs to machines that minimizes the communication cost, and the maximum job completion time, also known as the \emph{makespan}. 

\subsubsection{Joblet Size Estimation}
To estimate the size of a joblet, we must estimate the cardinality of the query path pattern $Q_k$.  We apply cardinality estimation techniques from query optimization over ontological queries~\cite{SRK07} that computes a probability distribution of the expected number of matches for each edge $(v_l,a_l,v_{l+1})$ in $Q_k$.  The distribution function provides a probability estimate of the number of matches of $v_{l+1}$, given the matches of $v_l$ connected via an edge $a_l$, satisfying the literals in $v_l$ and $v_{l+1}$. The estimation is computed based on the mean and standard deviation of the number of matches of $v_{l+1}$ w.r.t $v_l$~\cite{SRK07}.  We compute the distribution function of $Q_k$ as the product of the distribution functions of each consecutive edge in $Q_k$. We estimate the size of a job $|$\job$|$ \ as the cardinality of the query pattern $Q$, which is computed as the upper-bound of the minimum cardinality of all $Q_k$.  

%\textcolor{magenta}{Similarly, we estimate the number of matches for a job \job \ as the size of the job $|\mathcal{J}_{ij}|$ by computing the product of the distribution of each $Q_k \in Q$, where $Q$ is the pattern of $\sigma$\cite{SRK07}}.  
%\fei{I think this last statement should be the minimum cardinality among all $Q_k$ joblet sizes, as per page 15, 1st paragraph of the paper.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Detailed formula for reference
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\eat{
\begin{equation} \label{eq:jobletEstimation_mu}   \mu(v_l,v_{l+1})=\dfrac{1}{|v_l|}\sum_{a_l}  |(a_l, v_{l+1})|
\end{equation}
\begin{equation} \label{eq:jobletEstimation_VA}   \sigma^2(v_l,v_{l+1})=abs((\dfrac{1}{|v_l|}\sum_{a_l}  |(a_l, v_{l+1})|^2)-\mu^2(v_l,v_{l+1}))
\end{equation}
\begin{equation} \label{eq:jobletEstimation_VA}   D(v_l,v_{l+1})=\mu(v_l,v_{l+1})\pm k\sigma(v_l,v_{l+1})
\end{equation}
}
%\fei{This did not completely parse correctly for me, esp. the last sentence.  What is a distribution function?  Can you be more specific or provide a definition of the function?  A frequency count?  Please elaborate more on how this is done.} 
 %\fei{OK, the main message here is we define the size of joblet and job via these existing techniques by multiplying their functions.  I can shorten further after getting clarification of the above.}

\subsubsection{Communication Cost}
For a joblet \joblet, the fragment \fragment \ may contain a partial match of $Q_k$ over the induced subgraphs $G_t(v',d), t \leq i$, i.e.,\eat{with the query path $Q_k$ that resides in $M_j$ at timestamp $i$, the fragment $F_{ij}$ may only contain a partial match, i.e.,} some nodes and edges that match $Q_k$ reside in machine $M_{j'}, j' \neq j$.  We estimate the communication cost of a joblet, $CCost(\omega_{ijk})$, as the total number of such edges that must be transferred from all $M_j'$ to $M_j$, as  $CCost(\omega_{ijk})=\sum_{\substack{(v_1, v_2) \in G_t(v', d), \\ \neg((v_1, v_2) \in F_{ij})}}  |(v_1, v_2)|$.  This defines the communication cost of a joblet as the number of edges in $G_t(v', d)$ that are not in \fragment.   While we use query paths $Q_k$ to compute more accurate joblet size estimations, we assign \emph{jobs}, \job, to a machine $M_j$.  Hence, we define the communication cost of a job, $CCost(\mathcal{J}_{ij})=\sum_{\substack{k}} CCost(\omega_{ijk})$,  i.e.,  for $\sigma$ with pattern $Q$ on $M_j$, we aggregate over all the joblets containing the query paths $Q_k$ of $Q$.  


\eat{
\begin{equation} \label{eq:datashipment_Joblet}
  %  CCost(\omega_{ijk})=\sum|e(u_1,u_2)\in G_i(v',d)| \ \mid (u_1\not\in F_{ij} \lor u_2\not\in F_{ij})
   CCost(\omega_{ijk})=\sum_{\substack{(v_1, v_2) \in G_t(v', d), \\ \neg((v_1, v_2) \in F_{ij})}}  |(v_1, v_2)|  
\end{equation}
}
%Equation~\ref{eq:datashipment_Joblet}  

%\begin{equation} \label{eq:datashipment_Job}
%   CCost(\mathcal{J}_{ij})=\sum_{\substack{k}} CCost(\omega_{ijk})  
%\end{equation}

%\fei{Define for jobs as aggregation over joblets?}
%estimates the data shipment in terms of the number of edges for a given joblet along with its machine assignment. It counts the number of edges in the induced subgraph that has (at least) one end point not reside in $F_{ij}$. 

%***************************************************
%\subsection{Workload Assignment}\label{sec:WorkloadAssignment}

\subsubsection{Initial Workload Assignment} \label{sec:InitialWorkloadAssignment} We generate a job assignment among the worker machines such that the total communication cost $C$, and the makespan $\tau$ is minimized.  We do this by applying the pseudo-polynomial-time, 2-approximation algorithm by Shmoys and Tardos that solves the \emph{general assignment (GA) problem}~\cite{shmoys1993approximation}. Intuitively, given $C, \tau$, the GA problem is to find an assignment of each job $\mathcal{J}_{ij}$ to one of a set of parallel machines, taking time  $t_{\mathcal{J}_{ij}}$ \eat{=|\mathcal{J}_{ij}|}, and incurring cost \ccost$(\mathcal{J}_{ij})$ such that the total cost is at most $C$, and minimizes the makespan. Given lower and upper bounds $(t_l,t_u)$ for job runtimes, Shmoys and Tardos present a 2-approximation algorithm that computes a schedule with communication cost at most $C$, and makespan at most $2\tau$; as long as $t_l \leq t_{\mathcal{J}_{ij}} \leq t_u$.
%(twice the maat most  accepts a lower and upper bound $(t_l,t_u)$ for the runtime of each job and as long as the runtime of the job lies within this bound, the algorithm guarantees the 2-approximation. 
We assume these time bounds are given as input.  To find an assignment that is at most $2\tau$, the algorithm performs a bisection search on the range of possible makespan values by keeping only those assignments with an objective function value less than half of the objective function value of the best assignment found thus far.
The algorithm solves the linear program of the GA problem at most $log(wP)$ times, where $w$ is the total number of jobs and $P$ is the maximum workload among all jobs~\cite{shmoys1993approximation}. Among all the current assignments, we select the assignment with minimum makespan.
%%  that have makespan within the current range. \fei{The last sentence still hard to parse. "...with an objective function value less than half of the best assignment"?} \morteza{Please read my sentence again, I said "with an objective function value less than \textbf{half of the objective function value of the best current assignment}"}.\morteza{I put the original text of the algorithm in Figure\ref{fig:Clarification}, please feel free to revise.} 


%***************************************************
\subsection{Query Matching}
\label{sec:querymatch}

We discuss how query pattern matches are computed over a graph fragment, and then discuss how we maintain these matches in the presence of graph changes.  

%\fei{Need to give high level intuition first of how this matching is done, and then go into details.}
\stitle{Matching over Graph Fragments.} 
With a balanced workload assignment of jobs to machines, each $M_j$ executes the jobs \job \ to compute matches of each $Q_k$ corresponding to $Q$ over \fragment.  \eat{In this section, we explain how we match queries against the fragment using query paths.}  To avoid partial matches \fragment, the coordinator $M_{c}$ identifies edges that must be shipped to $M_j$, as defined by \ccost.  For each query path $Q_k$ in $\mathcal{J}_{ij}$, we perform subgraph isomorphism matching on \tempgraphk \ to find matches $h_i(\bar{x}_k)$, where $\bar{x}_k$ are literals in $Q_k$. For a given variable or literal $x \in \bar{x}$ in $Q$, we compute the matches of $Q$ over $x$ by taking the  intersection of matches across all query paths $Q_k$.  To find the matches of $Q$, we compute the union of matches for each variables and literals in $Q$~\cite{SRK07}.  

%we maintain information on each match and partial matches of each query path. To process the changes, we use these data structures to know if there exists a match and what changes can make a partial match to be a match.

%\fei{Edit as per our chat re. comment below.}
%Given a \job \ with a graph pattern $Q$ that contains a set of joblets \joblet \ for a candidate node $v'$ at snapshot $i$ on machine $j$, we find the matches of $Q[\bar{x}]$ on $\mathcal{G}(v',d)$.   To ensure we compute complete matches over a fragment \fragment, the coordinator $M_{c}$ identifies all edges that must be shipped to $M_j$, as defined by Equation~\ref{eq:datashipment_Joblet}.  \eat{How is this done?  How expensive is this?  The savings of not having to worry about partial matches comes at a cost.} \newtext{We assume the coordinator has access to an abstract graph of \tempgraph. This graph is smaller than \tempgraph \ by removing the attributes and only keep the edges and can be stored in the memory. Using the abstract graph, the coordinator is able to quickly identify the edges that needs to be shipped} For each query path $Q_k$ in $\mathcal{J}_{ij}$, we perform subgraph isomorphism on node $v'$ to find the matches $h_i(\bar{x}_k)$, where $x_k$ is the set of nodes in $Q_k$.  If there exists an $h_i(\bar{x}_k)=\emptyset$, it means that there exists no match for a query path of $Q$ on node $v'$,thus, there exists no match of $Q$. 


%In order to find the matches of $Q$, we compute the Cartesian product of the matches of all joblets, \emph{i.e.,} $h_i(\bar{x})=h_i(\bar{x}_1)\times \dots \times h_i(\bar{x}_m)$, where each $h_i(\bar{x}_k)\neq \emptyset$.   \fei{what does it mean to compute the product of matches?  What is the defn of this operation?  This differs from the cardinality estimation paper which uses intersection of all paths for a literal and the union of results across all literals/variables (Eqn.10).} 


%In order to keep track of the matches of the jobs, we initially define a boolean vector in the form of $\bar{\tau}_{v'}=(b_1,\dots, b_m)$ for each candidate node $v'$ of the job $\mathcal{J}$.  \fei{Is this not defined for each match of a query pattern $Q$ (per job)?} An entry in $\tau_{v'}$ could be either \emph{\underline{T}rue} or \emph{\underline{F}alse} and $b_k$ ($k \in (0,m)$) corresponds to the joblet $\omega_{ijk}$ with query path $Q_k$ of $\mathbf{J}_{ij}$. For each query path path $Q_k$, we also maintain an unsatisfied set of literals $\kw{unSat}_{v'}^k$ for a match of $v'$.  \fei{I'm confused when you say match of $v'$, are we not finding matches of $Q$ or $Q'$ in the induced subgraph around $v'$?}  For each query path $Q_k$, if we have a match $h_i(\bar{x}_k)\neq \emptyset$, then we set $b_k=T$, otherwise $b_k=F$. For a query path $Q_k$ with $b_k=F$, if there exists a match of the topology of $Q_k$ that does not satisfy some literals $x \in \bar{x}$, we set $\kw{unSat}_{v'}^k=(x)$.  \fei{What is $x$?} These vectors and sets will be used to maintain and find the new matches at the next snapshots. Details will be discussed on Section~\ref{sec:queryMatchWithChanges}. 

\begin{comment}
\fei{Few things to discuss: 
\begin{enumerate}
    \item refine notation, e.g., $h_i(x)$ is a function between query pattern and variables, not just query paths, careful with the use of $v$ in boolean vectors can be easily confused as a vertex\morteza{Changed to $\lambda$. Feel free to suggest your opinion if you think $\lambda$ is not good. Do you have any suggestion for the match of $Q_k$ instead of $h_i(Q_k)$? } 
    \item What does it mean to compute the cartesian product of a set of query matches?\morteza{It is to compute the matches of $Q$. Imagine you have 1 match for $Q_1$ and 2 matches for $Q_2$ and $Q_1$ and $Q_2$ are the query paths of $Q$. In this case, we have 2 matches of $Q$, which is a cartesian product of the matches of $Q_1$ and $Q_2$.}
    \item did not understand the role of empty match (empty set?).)\morteza{If there exists no match for a query path $Q_k$, then there exists no match for $Q$.}
    \item Need to give high level overview and use of an example, how many boolean vectors do you maintain?  What are their roles?  how are they used together to maintain your matchings?  How do they help \tedparallel to be more efficient (novelty)? \morteza{The details are discussed on Sec.~\ref{sec:queryMatchWithChanges}, Do you want me to discuss here? How we use them is based on changes coming to the fragment and we do not talk about those changes until Sec.\ref{sec:adaptive}.}
    \item We need to create an example here to show how this all works and better bring out the novel and impressive aspects.
\end{enumerate}
}
\end{comment}

%\subsubsection{Adapting to Changes}
%\label{sec:adaptive}


\stitle{Matching in the Presence of Graph Changes.}\label{sec:queryMatchWithChanges}
Incremental changes over \fragment \ can lead to the insertion and deletion of matches of $Q_k$.  To avoid repeated subgraph isomorphism computations in the presence of \fragment \ changes, we record partial matches for each $Q_k$ along with their missing topological and literal conditions.  

%To minimize the overhead of subgraph isomorphism operations as changes occur over fragments \fragment, 
We define boolean vector \vecmatchfull \ = $(b_1,\dots, b_{\kappa})$ over a candidate match \matchone \ of $Q$ in \fragment.  \vecmatchfull \ contains $\kappa$ components, where the $k$-th component represents the matching status of \joblet.  That is, if there exists a match \matchone \ of $Q_k$ in \fragment, then \vecmatchful \ = 1 (\kw{true}), otherwise, \vecmatchfull \ = 0 (\kw{false}).  In the latter case, a partial match \matchone \ may be isomorphic to  $Q_k$ but not satisfy its literals.  We define \unsatfull \ as the set of unsatisfied literals $x' \in \bar{x}$ in \matchone \ w.r.t. $Q_k$, i.e., \unsatfull \ = $\{x'.A = c| h_{t_i}({x'}).A \neq c\}$.  For brevity, we use  \vecmatch \ and \unsat \ when \matchone \ is clear from the context. 

Each machine $M_j$ initializes and populates \vecmatch \ and \unsat \ as matches are found.  As changes occur over fragments, \tedparallel \ uses \vecmatch, and \unsat to compute new matches, and updates  existing matches while minimizing the need for (expensive) subgraph isomorphism operations.  If the $k$-th component of \vecmatch \ equals \kw{false}, there are two cases to consider: (i) a topological match of $Q_k$ exists, but there exist unsatisfying literals in \unsat; and (ii) an empty \unsat \ represents no topological match of $Q_k$ in \fragment. For a given $\mathcal{J}_{ij}$, we consider the following cases for an input change $c$: 

\begin{enumerate}
\item[(a)] \uline{attribute insertion/deletion/update:} since there is no change in the topology in \fragment (no need for subgraph isomorphism operations), we check whether the new value in $c$ adds/removes literals from \unsat, and consequently, update \vecmatch \ to denote the insertion/deletion of a match \matchone \ w.r.t. $Q_k$.
\item[(b)] \uline{edge insertion:} we must perform a subgraph isomorphism matching to determine whether a partial match is upgraded to a complete match w.r.t. $Q_k$. 
\item[(c)] \uline{edge deletion:} an edge deletion in \fragment \ does not lead to new matches, but can cause a prior match \matchone \ w.r.t. $Q_k$ to be removed.  In this case, we set \vecmatch(\matchone)[$k$] \ to \kw{false}, and add any unsatisfying literals to \unsat(\matchone). 
\end{enumerate}

Algorithm~\ref{alg:LocalMatch} describes the details.  For attribute updates, we update \vecmatch \ and \unsat without performing any subgraph isomorphism operations (Lines 3-11). \eat{Removing an attribute cannot make a partial match to be a match, so it might only remove a match (Lines 9-11).} For edge insertions, we perform subgraph isomorphism along $Q_k$ to check for a new match (Lines 12-15). For edge deletions, which can only remove matches, we update $b_k$ for $Q_k$ \eat{However, removing an edge might only make a match to be disappeared and it is being handled by setting $b_k=0$, if necessary}(Lines 16-18). A match \matchone \ of $Q$ exists if $b_k=1$ for all $k$, and we add  \matchone \ to   \matchesJ{i} \ (Lines 19-21).

%After the first snapshot, $M_c$ sends the changes to the workers. Each worker needs to find/maintain the matches using the boolean vectors it initialized at the first snapshot. Algorithm~\ref{alg:LocalMatch} depicts how a change is applied on each machine to maintain/find the matches given the corresponding job and the previous matches. Given a job $\mathcal{J}_{ij}$, previous matches $\mathcal{M}_{t_{i-1}}$, a fragment $F_{ij}$ and a change $c$, $\kw{LMatch}$ find/maintain the matches by using the boolean vectors $\bar{\tau}$ and the set $\kw{unSat}$ of $\mathcal{M}_{t_{i-1}}$ and minimizing the call for subgraph isomorphism. If the change $c$ is add, update or remove an attribute, we do not perform subgraph isomorphism and use the value of $\bar{\tau}$ and $\kw{unSat}$ to perform the change (lines 3-12).  \fei{No change in topology, update the vector and unsat set acordingly.} If $c$ is to add a new edge, then we only perform subgraph isomorphism if it leads us to have a match for a joblet that contains the edge (lines 13-20).  \fei{subgraph iso. to identify new match from partial match or new match instance arises. (lines ab)}  Lastly, if $c$ is to remove an edge, we update the $\bar{\tau}$ and $\kw{unSat}$ accordingly \fei{if bit vector is 1 goes to 0, and update unsat set} without running subgraph isomorphism as removing an edge does not lead us to have a new match (lines 21-23).
%There exists a match $h_i(\bar{x})$ for a job $\mathcal{J}_{ij}$, if $b_k=1$ for each $k \in \bar{\tau}(h_{t_i}(\bar{x}))$  \fei{notation $k$ is a number} (lines 24-26). Using the $\bar{\tau}$ and the  set $\kw{unSat}$ helps us to keep track on \emph{why there exists/ does not exist a match for a $Q_k$} to avoid running subgraph isomorphism for each single change in the new snapshot.
%For example, knowing that we ignored a match at timestamp $i$ because of a literal $x.A=a$, we can quickly consider it as a match if $x.A=a$ is valid at timestamp $i+1$.  


\input{Algorithms/QueryMatching}

%At snapshot $i+1$, we process each change in the fragment based on the following conditions:

%\begin{itemize}
%    \item If the change is to add/update an attribute $x.A=a$ for a node $x$, and $x$ is part of a match $Q_k$:
%    \begin{enumerate}
%        \item If $b_k=0$ and $(x.A=a) \in \kw{unSat}^k$, then we remove $x.A=a$ from $\kw{unSat}^k$ and set $b_k=1$ if $\kw{unSat}^k=\emptyset$.
%        \item If $b_k=1$ and $x.A=b \in Q_k$ for $a\neq b$, then we add $x.A=b$ to $\kw{unSat}^k$ and set set $b_k=0$.
        %\item Otherwise, we apply the change. \fei{in cases where the update does not match the literal in $Q_k$
%    \end{enumerate}
%    \item If the change is to remove an attribute $x.A=a$ from a node $x$ and $b_k=1$, then we do as number (2) of the previous case. Otherwise, we apply the change.
%    \item If the change is to add an edge $e=(v_1,v_2)$;
%    \begin{enumerate}
%        \item If $e\in Q_k$ and $b_k=0$ for a vector $\bar{\tau}(h_{t_i}(\bar{x}))$, then we apply the change and perform subgraph isomorphism to evaluate $b_k$.
%        \item If $e\in Q_k$ and $b_k=1$ for all vectors $\bar{\tau}(h_{t_i}(\bar{x}))$, then we check if the new edge lead us to have a new match $Q_k$. In case of a new match, we duplicate the vectors and set $b_k=1$.
%    \end{enumerate}
%    \item If the change is to remove an edge $e=(v_1,v_2)$;
%    \begin{enumerate}
%        \item If $e\in Q_k$ and $b_k=1$ for a vector $\bar{\tau}(h_{t_i}(\bar{x}))$, then we set $b_k=0$ and set $\kw{unSat}^k=\emptyset$.
%        \item If $e\in Q_k$ and $b_k=0$, then apply the change.
%    \end{enumerate}
%\end{itemize}


\begin{example}\label{example:DefineVectors}
Figure~\ref{fig:matchingExample}(b) shows (partial) matches of query patterns $Q'_{1}, Q'_2$ (shown in (a)) for timestamps $t_{1}-t_{3}$.  At $t_1$, \vecmatch($h_{t_1}(\bar{x})$) \ denotes no match of either $Q_1$ nor $Q_2$, while  \vecmatch($h_{t_1}(\bar{x})$)[2] indicates a topological match of $Q_2$ with non-empty $\kw{unSat}_2$ containing literal $z=$ \lit{McMaster}.  At $t_2$, with an edge insertion labeled \lit{study} from \lit{Bob} to \lit{Waterloo}, we perform a subgraph isomorphism matching and find a topological match of $Q_1$.  However, \vecmatch(($h_{t_2}(\bar{x})$) remains  \kw{false} due to the unsatisfying \lit{McMaster} literal in $\kw{unSat}_{1}(h_{t_2}(\bar{x})$).  Lastly, the attribute value change at $t_3$ on \lit{University} from \lit{Waterloo} to \lit{McMaster} clears all unsatisfying literals, and updates \vecmatch($h_{t_3}(\bar{x})$) \ to \kw{true} for both $Q_1$ and $Q_2$, without requiring any additional matching.
 \end{example}

\eat{
\begin{example}\label{example:DefineVectors}
Continue with Example~\ref{example:QueryPath} and Figure~\ref{fig:matchingExample}(b), at timestamp $t_1$, $\bar{\tau}(h_{t_1}(\bar{x}))=(0,0)$ as there exists no match of $Q_1'$ and $Q_2'$ on the subgraph around the student $Bob$ in graph $G_{1}$. However, the $\kw{unSat}^{2}$ contains $z=`$\lit{McMaster}' as the university name is not satisfied, which means there exists a match of the topology of $Q_2'$. The unsatisfied set is empty for $Q_1'$ as there is no topological match of $Q_1'$.  \fei{This needs to be updated to reflect unsat for which match.}
%\fei{So in $Q_2$, the T in $\tau$ just means topological match?  We should remove the subscript on $\tau$ and replace with $\tau(h(x))$.}
\end{example}


\begin{example}
Continue with Example~\ref{example:DefineVectors} and Figure~\ref{fig:matchingExample}(b), in graph $G_2$ of timestamp $t_2$, a new edge is coming and it makes a match of the topology of $Q_1'$ after performing a subgraph isomorphism. However, the corresponding boolean in the $\bar{\tau}$ remains $0$ as $z=`$\lit{McMaster}' is an unsatisfied literal in $\kw{unSat}^1$. In graph $G_3$, the change in the department will be applied without any effects as there exists no literal on department name in $Q_1'$ and $Q_2'$. However, the change of the university to \lit{McMaster} would empty $\kw{unSat}^1$ and $\kw{unSat}^2$ without any subgraph isomorphism. As the unsatisfied set becomes empty, we set $\bar{\tau}=(1,1)$. There exists a match of $Q_3$ in $G_3$ over the entity \lit{Bob} as $\bar{\tau}(h_{t_3}(\bar{x}))=(1,1)$. 
\end{example}
}
%***********************

\subsection{Error Detection}
To compute \errorSigma, the error set for a set of \tgfds $\Sigma$, \tedparallel \ must: (i) compute the matches of $Q$ for each $\sigma \in \Sigma$, and (ii) validate $\sigma$.  In step (i), \tedparallel \ avoids partial matches across machines by copying the minimal number of nodes and edges between machines. \tedparallel then computes matches of $Q$ that are isomorphic to a subgraph of \fragment, which is done locally at each machine $M_j$ (via Algorithm~\ref{alg:LocalMatch}), as described in Section~\ref{sec:querymatch}.  

To validate each $\sigma \in \Sigma$, we evaluate matches that exist: (a) locally at each $M_j$, and (b) matches that occur across two (or more) machines $M_j, M_{j'}, j \neq j'$.  In case (a), matches \matchone \ and \matchtwo \ are evaluated similar to the single node case by executing the local error detection procedure \kw{LError} (Algorithm~\ref{alg:lError}).  These localized matches are then sent to the coordinator machine $M_c$, who annotates each \matchone \ with the originating machine $M_j$. The coordinator selects matches $h_{t_i}(\bar{x}), h_{t_{i'}}(\bar{x})$ from $M_j$, $M_{j'}, j \neq j'$, respectively, to validate.  This is done by selecting matches from $\mu_{X}(h_{t_i}) =$ \hashmapXY$(h_{t_i}$) and $\mu_{X}(h_{t_{i'}}) =$ \hashmapXY$(h_{t_{i'}}$) such that $|t_i - t_{i'}| \in \Delta$, and computing $\{\mu_{X}(h_{t_{i'}})\} \setminus \{\mu_{X}(h_{t_i})\}$  , i.e., checking whether the set difference is non-empty.  If so, we add $\{(h_{t_i}(\bar{x}), t_i), (h_{t_{i'}}(\bar{x}), t_{i'}) \}$ to the cross-machine error set \errorSigmaC.  At each timestamp $t_i$, we update \errorSigma += \errorSigmaC \ $\bigcup_j$ \errorSigmaJ.  %Algorithm~\ref{alg:localVio} and \ref{alg:tedparallel} provide the details. 

\input{Algorithms/LocalVio}

Algorithm~\ref{alg:localVio} provides details of the matching and local error detection at each $M_j$.  We compute matches and errors over the first graph snapshot $G_1$ (Lines 4-5), and then incrementally compute matches (Line 9), and errors (Line 10) via \kw{LMatch} and  \kw{LError}, respectively.  The set of local matches and errors for each $M_j$ are sent to $M_c$ (Line 11).  
Algorithm~\ref{alg:tedparallel} shows \tedparallel \ which first estimates the jobs and communication cost before assigning jobs to the machines (Lines 4-7).  At each $t_i$, $M_c$ sends the changes (computed from log files) to all machine workers.  Each $M_j$ runs Algorithm~\ref{alg:localVio} to compute matches and the local error set, which is sent to the coordintor node after each timestamp to minimize idle time at $M_c$ (Lines 8-11).  Lastly, $M_c$  computes errors between $M_j, M_j'$ by comparing matches from $M_j'$ (Line 13) with those from $M_j$ (Lines 14-15), and returns the total error set (Line 16).
%depicts the local error detection to be run on each machine $M_j$. On snapshot 1, $M_j$ finds the matches of each job by running subgraph isomorphism (Lines 3-5). For the other snapshots, $M_j$ first receives the changes from $M_c$ (Line 7) and then maintain the matches by calling the \kw{LMatch} algorithm (Line 10). $M_j$ then calls \kw{LError} to find the local violations (Line 11). After each snapshot, $M_j$ sends the matches and violation set to $M_c$ for the global error detection.}

\input{Algorithms/parallelTED}

%\newtext{Algorithm~\ref{alg:tedparallel} shows the execution of the \tedparallel algorithm. It is run on $M_c$ and works as a driver in our distributed setting. After initialization (Lines 1-3), it defines the set jobs for each \tgfd and estimate the size and communication cost (Lines 4-7). It then finds an assignment of jobs to machines in order to equally distribute the workload with minimum communication cost (recall the workload assignment of Section~\ref{sec:InitialWorkloadAssignment}) and sends the assigned jobs to the corresponding machines (Lines 8-9). Then, for each timestamp, $M_c$ sends the changes to the machines and then we run Algorithm~\ref{alg:localVio} on each machine $M_j$ locally to find the matches and local error set and then send back them to $M_c$ (Lines 11-15). \fei{make note} Next, $M_c$ find the global set of violations using \kw{LError} algorithm and filtering the matches that are from the same machine (Lines 16-18). The total set of violations can be computed after each snapshot (Line 19).}

\eat{
\fei{(1) This needs a few sentences to explain the overall execution of \tedparallel in Alg. 6.  Please update and shorten pseudocode to match notation and description above. \blue{Done.} (2)  I think you can remove GlobalVio and combine sub-parts of it into Alg. 6.  For ex. line 5 in GlobalVio is taken care of by selecting matches from different machines as I discuss above. In fact, localVio is just doing the same thing as LMatch and LError so you could remove this and add the main steps to Alg. 6 as well. \blue{Done.} (3)}}
%\fei{I assume that not all the matches have to be computed locally first before sent to $M_c$ to save time?  The current code seems to be this sequential case, but why not compute matches and send them to $M_c$ in batches/more frequently? (minimize idle time)} \blue{I send the matches to $M_c$ in batch after each snapshot. Is that what you mean?}
%(4) Note, that I re-use the local $\Pi$ structures, and just annotate with the originating machine in $M_c$.}
%\fei{Highlight your changes so I can clearly differentiate the new text.}

%Machine $M_j$ at each snapshot $i$, finds all the matches of the set of assigned jobs and detects the violations locally for the local matches. Using the error detection algorithm of Section~\ref{sec:incdetect}, the local set of errors $\mathcal{E}_j(F_{ij}, \Sigma)$ is computed on each machine $M_j$. Algorithm~\ref{alg:localVio} depicts how the local violation detection is done on a machine $M_j$. For the first snapshot, we simply run subgraph isomorphism for each assigned job and store the matches locally in \matchesJ{i} (lines 2-5).  \fei{careful with notation, subscript $j$ for machine, why not access matches via \matches with snapshot?}From snapshot 2 onwards, $M_j$ first receives the changes from the coordinator $M_c$ and then finds the matches by calling the $\kw{LMatch}$ function for each given change. After finding the matches, $M_j$ finds the local violation by calling the $\kw{LError}$ procedure of the Algorithm~\ref{alg:tedinc}. After each snapshot, each machine sends the matches to the $M_c$ for the global violation detection (line 13). 


%Algorithm~\ref{alg:GlobalVio} depicts the function to be run on $M_c$. To compute the errors that are caused by paring matches across the machines, $M_c$ first filters the matches that are from the same machine and then run the $\kw{LError}$ procedure of the Algorithm~\ref{alg:tedinc}. \fei{Is this the old text, what is the variant algorithm now?} The $\kw{LError}$ algorithm does not compare the matches of the same machine with each other. Note that the local error set $\mathcal{E}_j(F_{ij}, \Sigma)$ is computed without any interaction between machines as an error in $\mathcal{E}_j(F_{ij}, \Sigma)$ at snapshot $i$ is independent  of the existence of a match on another machine $M_k$. The errors across the machines are computed only in the $M_c$. \fei{Since you ship edges from one machine to another, you have a complete match on a machine, and the only item to consider is to compare matches at different timestamps from different machines - is that correct?  Trying to prune out what's known and focus on what's different.}
%At each timestamp during the error detection process, the set of all errors can be computed as \errorSigma $=\mathcal{E}_c + \bigcup_j(\mathcal{E}_j)$. To compute the complete error set of \tempgraph \ w.r.t $\Sigma$, we compute \errorSigma \ after all snapshots are processed.  \fei{It would be very nice to show in a figure the matches across 4 nodes, and local errors computed, using the $\Pi$ structures, and then how $M_C$ computes global errors. } \morteza{We have already shown how $\Pi$ works, what is the point of repeating that here?}

\begin{example}\label{example:TEDParallel}
Consider a \tgfd $\sigma$ with $\Delta = (0,3)$, two machines $M_1$, $M_2$, and coordinator $M_c$.  
Figure~\ref{fig:TEDParallel} shows matches \{$h_{t_1}$, $h_{t_4}$\} and \{$h'_{t_1}, h'_{t_5}$\} of $\sigma$ computed locally (via \kw{LMatch}) at $M_1$ and $M_2$, respectively.  $M_1$ computes local error set $\mathcal{E}_1$ by checking whether $\{h_{t_1}, h_{t_4}\} \models \sigma$. In contrast, $\mathcal{E}_{2} = \emptyset$ since $|t_5 - t_1| \not \in \Delta$.  $M_c$ receives all matches, and validates all pairs from differing machines, namely, $\{h_{t_1}, h'_{t_1}\}, \{h_{t_4}, h'_{t_1}\}, \{h_{t_4}, h'_{t_5}\}$.  Unsatisfying pairs are added to \errorsigma += $\mathcal{E}_c($\tempgraph, $\sigma$) $\bigcup \mathcal{E}_1$.
%Figure~\ref{fig:TEDParallel} shows how \tedparallel algorithm works over two workers $M_1$ and $M_2$, while $M_c$ coordinates the process. $M_1$ and $M_2$ finds the matches of the pattern of a \tgfd (not shown) with $\Delta=(1,3)$. $M_1$ finds $h_{t_1}$ and $h_{t_4}$ at $t_1$ and $t_4$ respectively, while $M_2$ finds $h'_{t_1}$ at $t_1$ and $h'_{t_5}$ at $t_5$. Both machines find their local error sets $\mathcal{E}_1$ and $\mathcal{E}_2$. 
%$M_1$ checks the pair $(h_{t_1},h_{t_4})$ as it's timestamp difference lies within $\Delta$ and $M_2$ does not have any valid pair as $(t_1,t_5) \not\in \Delta$ for the pair $(h'_{t_1},h'_{t_5})$. However, both machines send the matches to $M_c$ for the global error detection. $M_c$ filters the matches that came from the same machine and pair $(h'_{t_1},h_{t_4})$ and $(h_{t_4},h'_{t_5})$ to find the violations in $\mathcal{E}_c$. At the end, the total error set is computed as  \errorSigma $=\mathcal{E}_c + \mathcal{E}_1+ \mathcal{E}_2$.
\end{example}
 
 
%\fei{Can you be more specific here?  What is $M_c$ doing with these matches from two different machines?  You mention variant, is this different than the \tedincremental from Sec. 5?} \morteza{Yes, a variant that compare the matches that are received from different machines, as I mentioned. What has to be more specific?} 

%\fei{How is this different than \errorSigma?} \morteza{$\mathcal{E}_c$ is the set of errors for matches reside in different machines. It is explained in the previous sentence. I provided the formula on how to compute \errorSigma in the next sentence.} 

%\morteza{Local errors are stored in local error set $(\mathcal{E}_j)$. Global errors are computed in the set $(\mathcal{E}_c)$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
    \centering
    \includegraphics[scale=0.27]{figures/ParallelTED.png}
    \vspace{-0.3cm}
    \caption{Error detection in \tedparallel}
    \label{fig:TEDParallel}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%\input{Algorithms/GlobalVio}
%***************************************************



\stitle{Re-balancing the Workload.} 
Recall the initial workload assignment ensures the makespan is at most $2\tau$ provided that $t_l \leq t_{\mathcal{J}_{ij}} \leq t_u, \forall t_{\mathcal{J}_{ij}}$.   That is, the runtime for each job should lie within the given lower and upper bounds $(t_l,t_u)$.  As incoming changes occur over an induced subgraph  $G_i(v',d)$ in a \fragment, these changes can lead to an increased density of edges and matches that dis-proportionally increases the workload in \fragment \ relative to fragments in other machines.  This causes an imbalanced workload across all machines, and thereby increases the makespan $\tau$.  We define a \emph{burstiness time buffer}, \timebuff, representing the allowable (percentage) change in job runtime due to workload bursts.  For example, suppose we define \timebuff \ $= 5\%$, then we set $t'_{l} =$ ((1 - \timebuff) \ $\times \ t_{l})$, and $t'_{u} =$ ((1 + \timebuff) \ $\times \ t_{u})$ to represent the allowable time range $(t'_{l}, t'_{u})$ to account for the increased density and popularity of a new celebrity vertex.  For any job $\mathcal{J}_{ij}$, where $t_{\mathcal{J}_{ij}}$ lies beyond  $(t'_{l}, t'_{u})$, the coordinator $M_c$ detects such violations, and triggers a workload re-assignment that re-balances the workload across all machines.  We evaluate the overhead and frequency of workload re-assignments over real workloads in Section~\ref{}. \tbf We found for \tbf $\leq$ \timebuff $\leq$ \tbf, the overhead is \tbf and only \tbf re-assignments were triggered over \tbf timestamps with \tbf\% of changes. \fei{Morteza: please fill in when you have these experiments complete.}

%For snapshots $i\geq 2$, $M_c$ sends the changes of each joblet to the corresponding machines. The size of $\omega_{ijk}$ at snapshot $i$ ($i\geq 2$) is based on the number of changes happening on the induced subgraph $G_i(v',d)$ around $v'$. Each change will be applied to the corresponding induced subgraph and the matches will be maintained. \fei{this needs to be more precise. What does "around" the subgraph mean? Is it the number of changes affecting $G_{i}(v', d)$?  If so, how is this compatible with the number of matches of $Q_k$?  We are adding number of changes + number of matches?  Please explain and justify so I can understand and better revise.} \morteza{We need to process each change, no matter if it is leading a partial match to a match, or a match to a partial match, or a partial match to a partial match. In my opinion, the runtime is dependant to the number of changes.}

%After the initial job assignment and the first snapshot, $M_c$ sends the changes to each job for the new snapshot. However, we might see burstiness around a job that changes substantially compare to other jobs. For example, in a social network, one person might become a celebrity after some points in time and the subgraph around that person changes exponentially compare to other subgraphs. In this case, our initial workload assignment is imbalanced and we need to re-balance it. To detect the burstiness, we use the technique of~\cite{shmoys1993approximation} to assign a lower and upper bound of the allowed changes for each job. This can be specified as the input by the nature of the dataset. For example, one can specify $(0,10\%\times |\mathcal{J}_{ij}|)$ as the lower and upper bound, where it means that we are allowed to have changes from $0$ up to $10\%$ of the size of the job at each timestamp. Using this new setting, we initially assign the workloads with this lower and upper bound~\cite{shmoys1993approximation} with a 2-\emph{approximation} algorithm~\cite{shmoys1993approximation}. If $M_c$ detects a job that has changes more than the upper bound that leads us to violate the 2-\emph{approximation}, it triggers the workload re-balancing procedure to re-assign the workloads. 



%%%%%%%%%%%%%%\subsection{Optimizations}

%%%%%%%%%%%%%%Communication cost plays an important role in parallel distributed computation. Depends on initial fragmentation, \tedparallel might need to ship large amount of data from the first snapshot $G_1$ between machines. Although we minimize the communication cost in our assignment model, but still we do not have any control on the upper bound of the data shipment.In this section, we present a communication cost bounded of \tedparallel that performs error detection with bounded maximum data shipment.

%%%%%%%%%%%%%%\stitle{Adding a Maximum Cost to the Model.} To consider a maximum communication cost, we consider a \emph{user-defined} natural number $C$ as the maximum number of edges to be shipped between machines in the general assignment problem. We revise Equation~\ref{eq:generalassignment} and change the first statement as:
%%%%%%%%%%%%%%\begin{equation} \label{eq:revisedGeneralAssignment}
%%%%%%%%%%%%%%    \sum_{k=1}^{m}\sum_{i=1}^{n} Cost_{ki}\times X_{ki}\leq C
%%%%%%%%%%%%%%\end{equation}

%%%%%%%%%%%%%%Using Equation~\ref{eq:revisedGeneralAssignment}, we make sure that communication cost of the a \emph{feasible} assignment is less than $C$. If such an assignment does not exist, we need to do further optimization by grouping \tgfds and run the general assignment problem again. We repeat this process until we find a \emph{feasible} solution or no further grouping is possible.

%%%%%%%%%%%%%%\stitle{\tgfd Grouping.} Given a set of \tgfds $\Sigma$, we first aim to identify \tgfds that are correlated by accessing the similar types of nodes in the \tempgraph. For two \tgfds $\sigma_1$ and $\sigma_2$ with graph patterns $Q_1$ and $Q_2$ respectively, we compute the correlation as:

%%%%%%%%%%%%%%\begin{equation} \label{eq:patternCorrelation}
%%%%%%%%%%%%%%    argmax \sum_{e_1 \in Q_1} \sum_{e_2 \in Q_2} sim(e_1, e_2) 
%%%%%%%%%%%%%%\end{equation}

%%%%%%%%%%%%%%In Equation~\ref{eq:patternCorrelation}, the $sim()$ function checks if the two input edges have the same \emph{label} and the end points of the edges are from the same \emph{type}.  





 % Old text ******************************************************
\eat{
\fei{Discuss estimation of where matches may occur, i.e., which time intervals matches are likely to occur?  Induce an interval partitioning based on balancing workload across partitions.}

\textbf{Interval Partitioning}
As we visit each node $v_1 \in$ \component, in topological order, we retrieve the matches satisfying the literal conditions involving $v_{1}.\texttt{att}$.  As we visit each subsequent node $v_{2}$, matches from the working set are pruned based on whether they satisfy conditions involving  $v_{2}.\texttt{att}$.  After visiting all the nodes $v_i \in$ \component, $i = \{1 \ldots m\}$, we have a set of matches $\mathcal{H_{\mathcal{C}_S}}$ satisfying literals $X' \subseteq X$, where $\{v_{1}.\texttt{att}, v_{2}.\texttt{att}, \ldots v_{m}.\texttt{att}\} \in X'$.  For a \tgfd $\sigma$, if the retrieved matches thus far do not cover all the literals in $X$, then we will need to aggregate matches $\mathcal{H_{\mathcal{C}_S}}$ across the connected components to cover all literals in $X$.  For example, \fei{provide visual example showing a single $\sigma$ across multiple components.}

For component \component, let $\Sigma_{\mathcal{C}_{S}}$ be the set of \tgfds with $X$ attributes that overlap with attributes $v.\texttt{att}$ for $v \in$ \component.  To reduce the number of matches in our working set $\mathcal{H_{\mathcal{C}_S}}$, we prune all matches that lie beyond the largest upper bound, $q_{max}$, among all the time intervals $\Delta_i  = (p_i,q_i)$ belonging to $\sigma_i \in \Sigma_{\mathcal{C}_{S}}$, i.e., $q_{max} = \{q_i | max_{q_i}\{p_i, q_i\}, \Delta_i, \sigma_i \in \Sigma_{\mathcal{C}_{S}} \}$. 

For each \component, the set of matches $\mathcal{H_{\mathcal{C}_S}}$ represents a subset of matches that need to be verified for each $\sigma_i \in \Sigma_{\mathcal{C}_{S}}$.  Let  $\mathcal{H}_{\sigma_{i}}$ represent the set of matches from $\mathcal{H_{\mathcal{C}_S}}$ satisfying the literal conditions in $X$ w.r.t. $\sigma_i$. We can then retrieve the corresponding time intervals $\delta_{\sigma_i}$, where we must verify the dependency $X_i \rightarrow Y_i$ for each $\sigma_i$.  The time intervals for each $\delta_{\sigma_i}$ may overlap across the $\sigma_i$'s, as shown in Figure~\ref{fig:intervalsplit}.  To improve performance and parallelize the verification task, we exploit this temporal locality across the shared attributes by splitting the intervals across $n$ partitions.  

To achieve a good workload balancing across $n$ partitions, we seek an interval splitting over the temporal data that distributes the data such that no single partition is overloaded and becomes a bottleneck.  Le et. al., introduce the concept of \emph{optimal splitters} for temporal data, which induce a partition of the data, and guarantees that the size of maximum bucket is minimized among all configurations, given the number of desired buckets~\cite{LLTC13}.  The intuition is to avoid having any single partition store and process too many intervals, i.e., the size of the maximum bucket should be minimized. The goal is to find the bucket boundaries, known as \emph{splitters}, which split an interval into two intervals.   Given $|\Sigma_{\mathcal{C}_{S}}|$ \tgfds, a total of $N = |\cup \delta_i|$ time intervals for all $\sigma_i \in \Sigma_{\mathcal{C}_{S}}$, and $n$ buckets (partitions), the \texttt{OptSplit} algorithm finds optimal splitters in $O(N \cdot \log N)$~\cite{LLTC13}.  

\begin{figure}[tb]
	{\includegraphics[scale=0.8]{figures/intervalSplit.pdf}}
	\caption{Interval partitioning.}\label{fig:intervalsplit}
\end{figure}

\begin{example}
Consider Figure~\ref{fig:intervalsplit} that shows six intervals from two \tgfds $\sigma_1, \sigma_2$.  Recall that $\sigma_1, \sigma_2$ share overlap among the nodes $\{A, B, D\}$ in the (red) component from Figure~\ref{fig:graphPatterns}(a).  Given $n = 2$, with splitters $l_1, l_2$, this creates 3 buckets shown as $b_1, b_2, b_3$, with 3, 2, 2, intervals, respectively. A less optimal partitioning, shown via dashed lines yields 2, 3, 3, intervals.  
\end{example}
}

%**********************************************************************************************


==> prelim.tex <==
\subsection{Preliminaries}
\label{sec:prelim}
%We define temporal graphs, patterns, and necessary notation.

\stitle{Temporal Graph.}
%\label{sec:prelim_graphs}
%\fei{This is not consistent with our discussion with time, and needs to extend the above description. Morteza, please revise.} \morteza{I have revised the text to say that a temporal graph is a graph extended by time. But I do not know where is it inconsistent with description :( Could you please let me know what exactly to change?}
We consider a temporal graph as a sequence of graph snapshots, with fixed vertices $\mathcal{V}$ and possibly varying edges, and attribute values. Let \tempgraph \ be a temporal graph defined over a period of time, consisting of a sequence of graph snapshots $\{G_1, \ldots ,G_T\}.$  Each snapshot $G_T = (V_t, E_t, L_t, F_{A_t})$ at a timestamp $t \in [1, T]$ is a directed graph with: (i) a vertex set $V_t$; (ii) edge set $E_t = V_t \times V_t$; (iii) each node $v \in V_t$ (edge $e \in E_t$) has a label $L_t(v) (L_t(e))$ at time $t$; and (iv) for each vertex $v$, $F_{A_t}(v)$ is a tuple specifying the value for each attribute of $v$ at time $t$, i.e., a tuple of the form $(A_{1,t} = a_1, A_{2,t} = a_2, \ldots ,A_{n,t} = a_n)$, for attribute $A_{i,t}$ with constant $a_i$, representing the properties of vertex $v$ at time $t$.

%\textcolor{blue}{Furthermore, we assume a partial correspondence between graph snapshots is given. That is, for \snapshot, $G_{t+1}$, let $U_t \subset V_t$, $U_{t+1} \subset V_{t+1}$  be subsets of vertices that are known to be in correspondence. We refer to these as \emph{anchor nodes}  of \snapshot \ and $G_{t+1}$, respectively.  This can be modeled by adding artificial edges linking vertices across successive time points.  Such correspondences can be based on human input, or prior knowledge, and is intended to serve as an anchor for graph matching over time.}

\stitle{Graph Pattern.}
A graph pattern is a directed, connected graph $Q[\bar{x}] = (V_Q, E_Q, L_Q, \mu)$ containing a set of vertices $V_Q$ and edges $E_Q=V_Q\times V_Q$. For each node $v \in V_Q$ and each edge $e \in E_Q$, the function $L_Q$ assigns a label $L_Q(v)$ and $L_Q(e)$ to $v$ and $e$, respectively. Let $\bar{x}$ be a list of variables corresponding to the number of nodes in $V_Q$. Let $\mu$ be a function that maps each $v \in V_Q$ to a variable in $\bar{x}$. We access $x \in \bar{x}$ using $\mu(x)$, and use $\mu(x)$ and $x$ interchangeably.


\begin{example} \label{exm:patternsAndGraph}
%\fei{Complete example of temporal graphs with snapshots, fixed $V$ and patterns referring to Figure 1.}
For $Q_1$ in Figure~\ref{fig:mainExample}(a), $\mu$  maps \lit{patient, medication, disease} to $\{x, y, z\}$, respectively. $Q_2$ depicts a world leader ($x$) that is member of a party ($z$), and has a position ($y$) in a country ($w$).  Similarly, for $Q_3$, $\mu$  maps \lit{advisor, student,  department} and \lit{university} to $x$,$y$,$w$ and $z$, respectively. Consider $Q_{3}'$ with vertices \lit{advisor, student, university} and its corresponding edges. $Q_{3}'$ is embeddable in $Q_3$.
\eat{We return to Figure~\ref{fig:mainExample}(a), where (1) $Q_1$ is a pattern to capture a patient, where $\mu$ maps $x$, $y$ and $z$ to a patient, his/her disease and medication respectively;(2) $Q_2$ depicts a world leader ($x$) that is member of a party ($z$) and has a position ($y$) of a country ($w$); (3) Similarly for $Q_3$, $\mu$ maps advisor, student,  department and university to $x$,$y$,$w$ and $z$; (4) $Q_4$ is embeddable in $Q_3$ as there is an isomorphic mapping from $Q_4$ to a subgraph of $Q_3$ by removing department and its edges. 
Moreover, Figure~\ref{fig:mainExample}(b) depicts \tempgraph \ with $12$ snapshots. \tempgraph \ has a fixed set of vertices $\mathcal{V}$, where there exists instance of all entities at $t_1$ and all timestamps (removed entities for simplicity). If an entity is removed, all the incoming/outgoing edges of the vertex will be removed. At each timestamp $t_i$, the graph shows instances of the entities and how they change from the previous timestamps, \emph{e.g.,} \lit{Alice} being supervised by \lit{Prof. Brown} at time $t_3$ or \lit{Peter} is diagnosed with \lit{Flu} at $t_5$ and then takes \lit{tylenol} at $t_{8}$.}
\end{example}

Table~\ref{tab:symbols} summarizes our notation and symbols.
%, where (i) $T$ is a time window; (ii) $V_T$ is a set of nodes with a timestamp from $T$; (iii) $E_T \subseteq V_T \times V_T \times T$ is a set edges with $t \in T$.  Similar to graphs, for each node $v\in V_T$ (resp. edge $e \in E_T$), $L_T(v)$ (resp. $L_T(e)$) is a {\em type} (resp. an {\em edge label}) that exists at a timestamp $t \in T$.  Lastly, $F_T$ captures the sequence of attribute value pairs at a time in $T$.




% remove for now to avoid confusion with interval model
%A temporal graph \tempgraph \ may be expressed as a collection of snapshot graphs, $G_t=(V_t,E_t,L_t, F_t)$ at different timestamps $t \in T$.  A snapshot graph $G_t$ of \tempgraph \ is induced by the set of nodes and edges, and their corresponding labels and attributes at $t$.


%For each node $v$, $A(v,t)$ is a tuple $\{(v.A_1, a_1), \ldots (v.A_n, a_n)\}$ of attributes at $t \in T$. Each attribute has the same definition as in graphs. Each $A_i\in{\cal A}$, $i\in[1,n]$ is an attribute describing a node property that its value is denoted as $a_i$ while $A_i \neq A_j$ if $i \neq j$. Each pair $(v.A_i, a_i)$ states that the attribute $v.A_i$ = $a_i$. An edge $e=(v_1,v_2,t)(t \in T)$ encodes a link with a label $L(e,t)$ between $v_1$ and $v_2$ at timestamp $t$.

%Each node $v\in V$ has a unique identifier (e.g. \lit{URI} in many datasets) as $id(v)$ to uniquely identify the entity at each timestamp.

 %Each node (resp. edge) in $G_t$ has its own {\em type} (resp. {\em label}) and attributes at timestamp $t$. For a snapshot graph $G_t$, $|V_t|$ (resp. $|E_t|$) denotes the number of vertices (resp. edges) in $G_t$.



%**********************************************
\begin{table}
  \centering
  \caption{Notation and symbols.}
  \vspace{-3mm}
  \label{tab:symbols}
  \setlength\tabcolsep{2 pt}
  \small \begin{tabular}{l l}
  \toprule
    Symbol              & Description \\
    \midrule
%    $G_t, G'$  & snapshot graph at time $t$, subgraph  \\
    $G_t$, $G'_t$, \tempgraph & snapshot, subgraph, and temporal graph \\
    $Q[\bar{x}]$ & graph pattern \\
    $\sigma, \Sigma$ & single, and set of TGFDs \\
    $h_{t}(\bar{x})$ & match of $Q[\bar{x}]$ in \snapshot \ at time $t$ \\
   % $X,Y,y$ & LHS literals, RHS literals, RHS single literal\\
    \errorsigma, \errorSigma & violations of $\sigma, \Sigma$ in \tempgraph \\
    \matches & matches of $Q$ in \snapshot \\
    \intone, \inttwo & time domain of \matchone, \matchtwo \\
    \permissrange & permissable range of \matchone \\
    \hashmapX, \hashmapXY & matches with shared values in $X$, $XY$ \\
    \timehashmapX & timestamps of matches in \hashmapX  \\
    \mapfunc & returns \hashmapXY \ where $h_{t_{i}}$ belongs \\
    \bottomrule
    \end{tabular}
\end{table}


% ************************************************
% Graphs, Pattern Matching and GFD definitions
% ************************************************
\begin{comment}
% Saved for later reference if needed
\subsection{Graphs and Patterns}
We consider directed, attributed graphs $G = (V, E, L, F_A)$, where $V$ is a set of nodes, and $E \subseteq V \times V$ is a set of edges. For each node $v\in V$ (resp. edge $e\in E$), $L(v)$ (resp. $L(e)$) is a {\em type} 
(resp. a relation) from a finite alphabet $\tau$.  For each node $v$, its value is denoted as $v.$\val{val}, and is an example of an \emph{attribute} of $v$, describing a node property.  For each node $v$, its attributes $A_i\in\mathcal{A}$, $i\in[1,n]$ are captured in its \emph{property tuple}, $F_A(v)$, defined as a sequence of attribute-value pairs $\{(v.A_1, a_1), \ldots (v.A_n, a_n)\}$.  Each pair $(v.A_i, a_i)$ states that the attribute $v.A_i$ = $a_i$. 

A graph $G' = (V', E', L', F'_A)$ is a \emph{subgraph} of $G$ represented as $G' \subseteq G$ if $V' \subseteq V$ and $E' \subseteq E$.  For every node $v \in V'$ (resp. edge $e \in E')$ we expect the node (edge) labels and corresponding tuples to be equal to those from $G$, i.e., $L'(v) = L(v), F'(v)_A = F(v)_A$ ($L'(e) = L(e)$).



\stitle{Graph Pattern Matching.}
We adopt the same semantics for pattern matching as previous work~\cite{fan2016functional}. Given a graph $G$ and a graph pattern $Q[\bar{x}]$, a match is a subgraph $G' = (V', E', L', F'_A)$ of $G$ that is isomorphic to $Q[\bar{x}]$.  That is, there exists a bijective function $h$ from $V_Q$ to $V'$ such that for each node $u \in V_Q$, $L_Q(u)=L'(h(u))$. Similarly, $h$ maps $E_Q$ to $E'$ for each edge $e = (u, w) \in Q$ such that there is an edge $e' = (h(u), h(w))$ in $G'$ with $L_Q(e)=L'(e')$.  Moreover, $L_Q(u)=L'(h(u))$ always holds if $L_Q(u)$ is a wildcard ‘ ’.

\subsection{Graph Functional Dependencies}
%Functional dependencies as a mean of data quality have been extensively studied for relational data~\cite{fan2008conditional,fan2012foundations}. However, functional dependencies have been extended for graph data and a new class of dependency, called \emph{graph functional dependency} (\gfd) was proposed in~\cite{fan2016functional}. 
A \emph{graph functional dependency} (\gfd) $\phi=(Q[\bar{x}],X \rightarrow Y)$ contains a graph pattern $Q[\bar{x}]$ and a dependency $X \rightarrow Y$, where $X$ and $Y$ are sets of literals over variables in $\bar{x}$~\cite{fan2016functional}.  Specifically, a variable literal is of the form $x.A = y.B$, and constant literals $x.A=c$, where $x, y \in \bar{x}$, $A, B$ are attributes, and $c$ is a constant value.

The scope of $\phi$ is defined by the subgraph matches $h(\bar{x})$ to $Q$, and the dependency $X \rightarrow Y$ is applied to these subgraphs.  We say $h(\bar{x})$ satisfies $X$, denoted as 
$h(\bar{x}) \models X$, if all the literals in $X$ are satisfied.  A graph $G$ satisfies $\phi$, denoted as $G \models \phi$, if for \emph{all} matches $h(\bar{x})$ of $Q[\bar{x}]$ in $G$, if $h(\bar{x}) \models X$ then $h(\bar{x}) \models Y$.  Furthermore, a graph $G$ satisfies a set of GFDs $\Phi$ if for all $\phi \in \Phi$, $G \models \phi$.

%Fei: edited above for (1) diff. symbol for GFD vs. TGFD as per Table 1; (2) edited $h(x)$ is different than $h(\bar{x})$ below; (3) G satisfies *for all* not for any.

%Given a \gfd $\varphi=(Q[\bar{x}],X \rightarrow Y)$ and a match $h(\bar{x})$ of $Q[\bar{x}]$ in a graph $G$, we say $h(\bar{x})$ satisfies a variable literal $x.A=y.B$, if and only if, there exist two nodes $v=h(\bar{x})$ and $v^\prime=h(\bar{x})$ with two attributes $A$ and $B$ resp. and $v.A=v.B$; similarly for constant literal $x.A=c$. $h(\bar{x})$ satisfies $X$ of $\varphi$, denoted $h(\bar{x}) \models X$, if it satisfies all the variable and constant literals in $X$; similarly for $h(\bar{x}) \models X$. A graph $G$ satisfies a \gfd $\varphi$, denoted as $G \models \varphi$, if for any match $h(\bar{x})$ of $Q[\bar{x}]$ in $G$, if $h(\bar{x}) \models X$ then $h(\bar{x}) \models Y$.
\end{comment}

==> response.tex <==
\twocolumn
\pagenumbering{gobble}

\section*{\textbf{Inconsistency Detection with Temporal Graph Functional Dependencies}}
\begin{center}\textbf{Response Letter \\
(Paper ID: 536, revision of paper \#9)}
\end{center}
\label{sec-response}
%\vspace{1.8ex}

We thank the reviewers for their thorough and constructive comments to improve this work.  We address all comments and highlight our changes in \reviseOne{blue} in the revised manuscript.

\label{sec-response}
%\vspace{1.8ex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{1.8ex} \hrule \vspace{0.6ex} 
\noindent {\bf REVIEWER 1.}

\noindent{\bf R1.O1} {\em Figure~\ref{fig:mainExample} is hard (or too complicated) to read. Either simplify it or add more explanations.}

\noindent{\bf [A]} We simplified Figure~\ref{fig:mainExample} for improved readability.  (1) We removed query pattern $Q'$ and showed its relationship to the original pattern $Q$.   (2) We removed the duplicate match at $t_2$ (but marked its continuous existence).  (3) We separated graph pattern $Q$ (a) from its temporal matches (b), and updated the Example~\ref{fig:mainExample} text accordingly.

\noindent{\bf R1.O2} {\em For the parallel \tgfd error detection. What about piggybacking existing distributed graph systems such as GraphX or GRAPE.}

\noindent{\bf [A]} 
This is an insightful comment.  GraphX provides a general purpose API for parallel graph computation with flexible data views, and standard graph algorithms.  However, it was not designed to support efficient graph pattern queries, i.e., computing simple subgraphs isomorphic to a query pattern $Q$ requires external libraries such as GraphFrames~\cite{graphframes}.  GraphX also does not include temporal operators to support incremental maintenance of query matches over dynamic graphs.  Exploring how changed vertices and edges can be integrated with GraphX to support incremental and localized subgraph matching for our error detection task is an interesting avenue of future work.

GRAPE parallelizes sequential graph algorithms based on a simultaneous fixed point computation via partial evaluation (PEval) and incremental evaluation (IncEval) phases~\cite{FXW+17}.  Despite providing native programs for subgraph isomorphism, GRAPE requires its PEval and IncEval phases to satisfy a monotonic condition, i.e., changes to the update parameters must adhere to a partial order defined over its variable domain.   While this property may hold for many graph computations (e.g., single shortest paths), it is not necessarily true for incremental pattern matching over dynamic graphs.  This limits the applicability of GRAPE for TGFD error detection. 


%\fei{Yinghui?  Add discussion to related work and in Section IV of why existing methods not sufficient?}
%**********************
\noindent{\bf R1.O3} {\em What is the time complexity of Algorithm~\ref{alg:tedparallel}?}

\noindent{\bf [A]}  In Algorithm~\ref{alg:tedparallel}, \kw{GenAssign} runs in polynomial time taking at most $2\tau$ to assign joblets~\cite{shmoys1993approximation}.  The initial subgraph matching dominates the runtime (\kw{LocalVio}) as  an exponential number of subgraphs may match $Q$ for each $\sigma$.  Fortunately, subsequent, incremental matching takes linear time proportional to the number of changes at each worker due to our $K$-Path decomposition.  Since $|Q|$ is small in practice, and we localize the matching to small graphs making it less likely to find exponentially many isomorphic subgraphs.  At each superstep $t$, incremental violation detection (\kw{IncTED}) runs in linear time w.r.t. the number of matches in \snapshot.   We add the above \emph{Runtime Analysis} discussion to the end of Section~\ref{sec:parallel}.


\noindent{\bf R1.O4} {\em In Experimental section Figure~\ref{fig-efficiency}, the run time of \gfdbasic is close to \tedparallel. Hence, the question is whether \gfdbasic is good enough in practice?}

\noindent{\bf [A]}
\gfds model a different dependency semantics that does not include the time intervals of when a graph pattern and a dependency should hold.  Practical applications with time independent graph FDs can still use \tedparallel since \tgfds  reduce to \gfds for time intervals of zero.  While \tedparallel shows modest gains over \gfdbasic when $T$ is small (e.g., over \dbpedia), we note that \tedparallel achieves significant F1-accuracy gains (up to 55\%) and 20\% improved runtime as $T$ increases (up to 38 timestamps in \imdb) due to the increased number of pairwise comparisons.  \gfdbasic does not include pairwise comparisons \emph{across} timestamps, i.e., in practice, it is unable to identify violations induced by a time period.

\noindent{\bf R1.O5} {\em Section~\ref{sec:caseStudy} Case Study is interesting. Can you provide more cases, which might be more useful than showing scalability by varying different parameters on synthetic datasets?}

\noindent{\bf [A]} We include two additional case study examples using a new \emph{Patient-Drug-Disease (\pdd)} dataset~\cite{wang2017pdd} (Section~\ref{sec:caseStudy}).  The two new TGFDs show for a given patient, disease, drug, we find inconsistencies in the administered dosage and the frequency duration.  Identifying such violations is  critical to ensure treatment efficacy.  For example, we found 21\% of hypertension patients taking \lit{Metoprolol}, were doing so with inconsistent dosages ranging between 5mg to 100mg.  Similarly, our \tgfds found that 41\% of patients were taking their medication over an irregular duration of days.  \eat{Lastly, our algorithms identified drug  \lit{Furosemide}, and \lit{Hypertension} as being the most erroneous drug and disease, respectively, occurring over 29 (out of 31) days.}  Identifying such violations is the first step towards correcting and regularizing drug treatment protocols.  We include \tgfd definitions and details in Section~\ref{sec:caseStudy}.


%states that for a given disease, patient and drug, we expect a consistent dosage to be administered for treatment efficacy.  Specifically,  we found that for the group of 1323 patients that suffer hypertension, 21\% were taking inconsistent dosages of the drug \lit{Metoprolol} (with drug bank id \lit{db00264}) between 5-100mg.  In TGFD4, For a given patient, disease, drug, and dosage, we found that 41\% of patients were taking their drug dosage over inconsistent duration days, \eg 0-14 days.  
%Lastly, we found \lit{Furosemide} (with drug bank id \lit{db00695}) and Hypertension  as the most erroneous drug and disease, respectively, occurring over 29 (out of 31) time intervals.

%\morteza{We plan to provide more case study from \pdd dataset.}
%\fei{Include 2 cases studies, with statistics on pct of errors, and most erroneous values (drug/disease).  }
%\fei{Make sure to add PDD dataset description to Section V.A.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{1.8ex} \hrule \vspace{0.6ex} 
\noindent {\bf REVIEWER 2.}

\noindent{\bf R2.O1} {\em It is unclear how the discovered \tgfds (e.g., minimality, thresholds used during discovery) will affect error detection. That is, the paper referred to \tgfd discovery to~\cite{NoronhaC21} and assumed that the “perfect” set of dependencies is given. However, an FD discovery procedure usually finds multiple candidates and does the pruning. I expect to see a discussion to connect the \tgfd discovery to using \tgfd for inconsistency detection, which should clarify whether it is practically possible to use the discovered set of \tgfds for error detection. For instance, is it easy to find the minimal set of \tgfds given the input data? If not, can you still make the error detection efficient for large graphs?}

\noindent{\bf [A]}
In practice, we expect that data designers will define a set of (curated) TGFDs according to their domain semantics, and application requirements.  In the absence of such predefined TGFDs, we mine minimal and frequent $k$-bounded TGFDs~\cite{NC01}.  The input parameter $k$ defines the maximum size (in edges) of  discovered graph patterns, and frequency is defined as satisfying a given support threshold.  We prune redundant, non-minimal candidates (those containing  embedded TGFDs), and infrequent candidates not satisfying the support threshold.   

We set the support level to find approximate TGFDs, which allow for exceptions.  From these exceptions, we consider matches with the most frequent consequent values as the ground truth, and the remaining consequent (exception) values as errors in the \tedparallel error detection.  Naturally, lower support values lead to more exceptions and more errors.   Larger $k$ values lead to a larger number of TGFDs with greater expressiveness involving more literals.

% double check with Levin for support of 1% is pattern support or TGFD support.  Removed for now, and reporting only k is awkward. 
As correctly noted by the reviewer, a large number of TGFDs may be returned and selection strategies, which often require domain expertise, are needed to define the initial set.  In our case, we discovered 100 (\dbpedia), and 80 (\imdb) \tgfds.  We select the top-40 TGFDs (based on decreasing support) as our initial set.   Other ranking measures such as the time window where a \tgfd holds, or the cardinality of the exception domain may also be used as a selection metric. We perform this selection offline as a preprocessing step.  Careful consideration is needed to identify reliable \tgfds (high support), and filtering `accidental' \tgfds, which are overfitted to the data, and are less meaningful (tuning $k$, and via the ranking measure).  Our method achieves these goals by allowing users to tune support, and $k$, and to apply post-discovery ranking metrics according to the application requirements.  We update Section~\ref{sec:expsetup}/TGFDs Generation, to reflect the above discussion.

%Lastly, given the dynamic nature of temporal graphs, as updates occur, mining a new set of TGFDs from scratch is infeasible.   As next steps, we intend to explore cleaning algorithms to update the temporal graph \tempgraph \ and/or the set of TGFDs , as they may become stale and realignment with the data becomes necessary. 


\noindent{\bf R2.O2} {\em The remarks and comparison between \tgfds and \gfds are sufficient. It will improve the paper if the comparison/remark between \tgfd and functional dependencies over temporal databases are added. For instance, is it feasible to transform the temporal graphs to relational data and then use the temporal extensions of \fds or relaxed \fds? It would be nice to see such a discussion, e.g., in the related works.}

\noindent{\bf [A]}
We add a new related work subsection \emph{Temporal Dependencies} (Section~\ref{sec:rw}) to discuss the relationship between \tgfds, and FDs over temporal databases, namely 
\emph{Dynamic Functional Dependencies (DFDs)}~\cite{JSS96}, and \emph{Temporal Functional Dependencies (TFDs)}~\cite{ WijsenVO93}.  DFDs are defined to hold over consecutive snapshots (states) of a database, where attribute values from a current state determine values in the next state, e.g., a new salary is determined by the last salary and the last merit increase.  TFDs rely on object identity, include a valid-time on tuples,  and apply to the sequence of snapshots defining a temporal relation~\cite{WijsenVO93}. DFDs constrain pairs of adjacent states, while TFDs constrain a sequence of multiple valid-time states.  \tgfds impose topological constraints that are not captured in relational settings, and \tgfds model a different matching and temporal semantics.  DFDs and TFDs impose consistency over tuples from adjacent snapshots, whereas \tgfds constrain the time difference of  matches to lie within the $\Delta$ time interval.  \tgfds model the time interval duration when topological and attribute consistency is expected, whereas DFDs and TFDs do not model such semantics.  

%\fei{ Schemaless  vs. fixed schema, inclusion of nulls resulting in lower accuracy.}


\noindent{\bf R2.O3} {\em The accuracy results in Section~\ref{sec:accuracyExperiments} are thin, given only two datasets are tested. The authors should evaluate their approach over more datasets to show that performance improvement is general.}

\noindent{\bf [A]} 
We update Section~\ref{sec:accuracyExperiments}, and now include the accuracy results for the \dbpedia dataset (Figure~\ref{fig:f1(dbpedia)}).  We also add a new comparative accuracy experiment using the \emph{Patient-Drug-Disease} (\pdd) dataset~\cite{wang2017pdd} (Figure~\ref{fig:f1(pdd)}). Over all three datasets, \tedparallel consistently achieves higher F1-accuracy over the baselines, i.e., between 20-60\% gain over \gfdbasic, and between 48-74\% gain over \gtarSubIso.  We also show \tedparallel achieves lower runtimes than \gfdbasic and \gtarSubIso on \imdb by (32\%,  119\%) (Figure\ref{fig:f1runtime(imdb)}), \dbpedia (67\%, 140\%), and \pdd (73\%, 151\%), respectively.  
Runtime graphs for \dbpedia and \pdd can be found in~\cite{AMCW21}

%\morteza{I brought back the accuracy results over the \dbpedia dataset. we planned to run the similar test over \pdd dataset}
%\fei{Can you please update the text in the paper in blue, and write a draft response here? Thanks.} \morteza{Done.}

%\fei{include 6 graphs (1 F1-accuracy, 1 runtime) for each dataset (PDD, IMDB, DBPedia) over 3 algorithms (GFD, GTAR, TGFD)}

\noindent{\bf R2.Q10}
Please provide more and clearer navigation on how to find the exact sets of TGFDs used for each experiment, corresponding to TABLE 2. Also, downloading the dataset now requires access. It would be nice to provide more examples of the error set of each dataset.

\noindent{\bf [A]} 
We update the Github site~\cite{datasite} (Section 2.1) to describe how to use the TGFDs defined in /sampleTGFDs/, and add a new figure visualizing a \tgfd with the corresponding syntax.  We include a new link to download all the datasets (/Dataset/README.md), and provide example errors for each of the four datasets (Section 2.2).  

%\fei{IMDB and Synthetic error files in /sampleResults/?} \morteza{Done.}


%OK.  Please update here when all is done, thanks.
%\begin{enumerate}
%    \item /sampleResults/ shows /DBpedia and /PDD.  Are there sample violations for /IMDB and /synthetic?  PDD violation file cannot be opened. \morteza{\imdb is running and will be done soon. Next, I will run \synthetic. All will be done by tonight. \pdd file was large and needed to be downloaded to view. I uploaded a smaller file for another pattern with fewer inconsistencies.} I am on my way to the lab to finish the synthetic test and upload the data.
%\end{enumerate}

%\fei{Morteza, please confirm if all of the above done. } \morteza{Done with example. However, I need to run one \tgfd error detection for \dbpedia, \imdb, and \synthetic and provide the violation file in the /sampleResult/. Right now, I have added an example file for the \pdd dataset. The reason is the format of the report has changed recently to be more human readable (as in the current result for \pdd) and I need to generate the violations in the new format to be consistent, so I need to run the test for at least one \tgfd for each dataset.}
%\fei{What happened to Section 2.1 and the TGFD picture on the Github site?  Please add Sec. 2.1 and 2.2 as we discussed when you have all the results. Update the dataset download link (still showing google drive). Thanks.} \morteza{This~\cite{datasite} is updated and everything is added. I have been updating this since a few days ago. I guess you might have been looking at mac-dsl repo. I imported the project on this repo to reflect the lates changes.}

%\fei{Update TGFD generation process, upload datasets to OneDrive, update Github links, check link availability, Section 2.1 in Github "TGFD setup" showing steps, Sec. 2.2: Example errors.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{1.8ex} \hrule \vspace{0.6ex} 
\noindent {\bf REVIEWER 3.}

\noindent{\bf R3.O1} {\em It would be beneficial to get an insight on how important the problem is. \tgfd defines just one class of functional dependencies in temporal graph. One possibility is to perform a study of inconsistency checks on graphs and evaluate the amount of checks that can be defined using \tgfd.}

\noindent{\bf [A]} Closest to our work, temporal association rules (\gtars), and \gfds, model time induced, frequent graph patterns, and FD semantics over graphs, respectively~\cite{namaki2017discovering, fan2016functional}.  As suggested, we analyzed the violations of \tgfd3 using \pdd from Section~\ref{sec:caseStudy}, and found 7671 inconsistencies.  Assuming a fixed graph pattern, we defined a \gtar using the most frequent drug \lit{Glucose} (drug id \lit{db09341}) and dosage \lit{250mL}, capturing 312 matches, but missing 719 (or 70\%) of the violations.  This loss is due to (1) \gtar's inability to compare against ``past" matches; and (2) \gtars impose only an upper bound of the time interval, leading to an increased number of matches and false positives (FPs).  We observed this latter case when \tgfds, with more selective (lower-bounded) time intervals had no FPs compared to 56 FPs with \gtars.  We found 60\% of inconsistencies occurred \emph{across a time interval}, which were missed by \gfds.  Only 40\% of the violations occurred over a single graph snapshot, thereby demonstrating the utility of \tgfds, and the prevalence of inconsistencies \emph{across time}.   We update Section~\ref{sec:accuracyExperiments} to reflect the above.
%\fei{Morteza: please update the above for errors within a snapshot, and across timestamps.  Also update Section~\ref{sec:accuracyExperiments}.} \morteza{Working on it.}

%Using \pdd dataset, we analyzed the violations of \tgfd 3 of the case study (). In total, we have found 7671 inconsistencies, in which 1031 of the inconsistencies were using different dosage of the drug \lit{Glucose} (drug bank id \lit{db09341}). The most common dose of this drug was \lit{250ml}. We created a \gtar based on the constant value of the drug name (\lit{Glucose}) and the most common dose (\lit{250ml}). The \gtar was able capture 312 consistent occurrences of this drug dosage, while missed the 719 inconsistencies, which forms only 30\% of the violations. However, \tgfd was able to capture all the inconsistencies. Moreover, \gtar is limited to capture the pairs that their time difference is less than the $\Delta$ value (in this case 7 days), while \tgfd only captures those with time difference within the $\Delta$ value (\ie 1 to 7 days). The interval limitation caused \gtar to capture 56 false positive pairs, while we had no false positive in \tgfd.
%\fei{How many errors occurred in a single timestamp, i.e., GFDs?}

%\morteza{find the errors of a TGFD over a real world graph, \eg \dbpedia, then for an entity with the same values on the LHS, check the most common value on the RHS and create a \gtar based on that. Given that, we can provide statistics on inconsistencies that can be captured by \tgfds, but not \gtars.}

%\fei{Morteza: please write a response here based on your evaluation results.  We can then add a summary of these results to Section~\ref{sec:accuracyExperiments}.} \morteza{Done.}

\noindent{\bf R3.O2} {\em There are a few typos in the paper. Please refer to 11 for more details.}

\noindent{\bf [A]} Thank you for pointing these out.  We have carefully reviewed the paper and fixed the typos.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{1.8ex} \hrule \vspace{0.6ex} 

\reviseOne{}

\reviseTwo{}




==> singleTGFD.tex <==
%**********************************************************************************************
\subsection{Single \tgfd} \label{sec:singleTGFD}

%By associating nodes, edges to the time intervals $\{\delta_1, \ldots \delta_k\}$ where specific properties hold, we can retrieve matches that share the same topology (following subgraph isomorphism of $Q$ against \tempgraph), and share the same attributes and values satisfying given predicates $x \in X, Y$.  This simplifies the matching process to quickly identify matching entities and their corresponding time intervals rather than checking each individual entity at a time.  

\begin{figure*}[tb]
	\includegraphics[scale=0.55]{figures/TEDexample.png}
	\vspace{-2ex}
	\caption{(a) Temporal graph and graph patterns. (b) Matched values in $\upsilon_X, \upsilon_{XY}$ are shown with their $\delta(X), \delta(XY)$ intervals, respectively.
	%\fei{The correlations between (a) and (b) need to be more obvious. Suggest linear timeline; highlight the X values (e1, e2) in (a); show the continuity of $\upsilon_{X21}$ matches. You can decrease the size of this graph.}
	}\label{fig:TEDexample}
	\vspace{-1ex}
\end{figure*}


Using intervals, we discuss error detection for a single \tgfd $\sigma$, and then present our algorithm for handling multiple \tgfds. In the latter case, we leverage shared topology and attributes to reduce the matching cost among a set of \tgfds, and apply interval splitting techniques to parallelize the error detection task among a set of partitions.  We first introduce required notions. 

Let $e$ denote an entity in \tempgraph \ with associated attributes and values. For $\sigma = (Q[\bar{x}],\Delta, X \rightarrow Y)$, let $\upsilon_X$ represent the set of matches partitioned according to their values in $X$, i.e., $\upsilon_X = \{(h_{t_i}(\bar{x}),  h_{t_j}(\bar{x})) | (h_{t_i}({x}).A = h_{t_j}({x}).A)  \lor (h_{t_i}({x}).A = a), \forall A \in X\}$, for constant $a$.  Similarly,  let $\upsilon_{XY}$ represent a sub-partitioning of matches in $\upsilon_X$ that share the same values in attribute $Y$, i.e.,  $\upsilon_{XY}$  = $\{(h_{t_i}(\bar{x}), h_{t_j}(\bar{x})) | (h_{t_i}({x}).Y = h_{t_j}({x}).Y) \lor (h_{t_i}({x}).Y = b), \{h_{t_i}(\bar{x}),  h_{t_j}(\bar{x})\} \in \upsilon_X\}$, for constant value $b$.  

For each $\upsilon_X$ ($\upsilon_{XY}$), there exists an interval, $\delta(X)$ ($\delta(XY)$), representing the time interval where the unique values in $X$ ($XY$) hold in \tempgraph.  Without loss of generality, we assume that the matches $\upsilon_X$ ($\upsilon_{XY}$) and their corresponding intervals $\delta(X)$ ($\delta(XY)$) are associated to an entity $e$; effectively capturing the evolution of $e$ over time.  Figure~\ref{fig:TEDexample}(b) depicts these notions.  

\begin{example} \label{ex:singleTGFD1}
Figure~\ref{fig:TEDexample}(a) shows \tempgraph \ with two player matches $e_1, e_2$ w.r.t. $\sigma = Q_1[w, x,y,z], (0,6\ months), (x_{t_i}=x_{t_j} \land w_{t_i}=w_{t_j} \land z_{t_i}=z_{t_j} \rightarrow y_{t_i}=y_{t_j})$.  Figure~\ref{fig:TEDexample}(b) shows that matches for $e_1$ with $\upsilon_{X_{11}}, \upsilon_{X_{12}}$ correspond to values in $X$ as \{\lit{Toni Kroos, La Liga, Real Madrid CF} \} and \{\lit{Kroos, La Liga, Real Madrid CF}\}, respectively.  At Dec. 2019, $e_1$ changes his number, leading to $\delta(X_{11})$ mapping to $\delta(X_{11}Y_{1}) = [Sep.2019, Nov.2019]$, and  $\delta(X_{11}Y_{2}) = [Dec.2019, Jan.2020]$.  
\end{example} 

%\morteza{I have revised this paragraph according to our latest call.}

We proceed with error detection for a single $\sigma$ as follows.  First, we compute $\upsilon_X$, i.e., $(h_{t_i}(\bar{x}), h_{t_j}(\bar{x})) \in \upsilon_X$ satisfying $Q[\bar{x}]$ in \tempgraph, and by definition, matches not satisfying defined constant literals in $X$ are discarded.  Second, for each $\upsilon_X$, there exists a $\delta(X)$ representing the time interval where the values in $X$ hold.  For each $\delta(X)$, there exists one or more intervals $\delta_{XY}$, corresponding to the time intervals where unique values in $XY$ hold. \newText{We check whether the corresponding $\delta(XY)$ of $\upsilon_{XY}$ lies within $\Delta$, i.e., $|\delta(XY)| \in \Delta$.  If not, these matches in $\upsilon_{XY}$ are removed. } %\newText{If there exists no interval $\delta'_{XY}\in \delta_{XY}$ such that $\delta'_{XY}$ lies within $\Delta$, then the matches in $\upsilon_X$ are removed.  FC: Are you looking for sub-intervals or do you just want to check $|\delta(XY)|$?} 
%\morteza{$\delta(X)$ is one time interval corresponding $\upsilon_X$. however, $\delta(XY)$ could be a `set' of time intervals. If a time interval in $\delta(XY)$ doesn't lie within $\Delta$, then we can remove it from $\delta(XY)$. If all the time intervals are removed from $\delta(XY)$, the $\upsilon_X$ can be removed.} 
%\fei{$\delta(XY)$ represents a time interval corresponding to a unique set of values in XY, so it is just one time interval.  For a given $X$, yes, there can be multiple $\delta(XY)$ intervals.  I think you can achieve what you want with checking if $|\delta(XY)| \in \Delta$.}
Third, for the remaining matches $(h_{t_i}(\bar{x}), h_{t_j}(\bar{x}))$ in $\upsilon_X$, we check whether $(h_{t_i}(\bar{x}), h_{t_j}(\bar{x})) \models Y$.  Since $\sigma$ is in normal form, $Y$ either contains a constant literal $y_{t_i}.A = a$, or a variable literal $y_{t_i}.A = y_{t_j}.B$.  If $Y$ contains a constant literal, and  $(h_{t_i}(\bar{x}), h_{t_j}(\bar{x})) \not \models Y$ for $(h_{t_i}(\bar{x}), h_{t_j}(\bar{x})) \in \upsilon_{XY}$, then we add matches in $\upsilon_X$ to \errorsigma.  Alternatively, if $Y$ contains a variable literal, then we check whether matches in each $\upsilon_X$ correspond to different values in $Y$, and if so, an error exists.  If there exists a single $\delta(XY)$, i.e.,  $\delta(X) = \delta(XY)$, then there is no violation.  However, if a $\delta(X)$ `splits' into two or more intervals $\delta_i(XY), i \geq 2$, then a change in the $Y$ value has occurred at the time point between two intervals, leading to an violation.  Hence, we add the corresponding $(h_{t_i}(\bar{x}), h_{t_j}(\bar{x})) \in \upsilon_X$ to \errorsigma.

%%%%%%%%
%% Dr. Chiang's paragraph regarding the error detection process. In this paragraph, we discard only based on \delta(X), which had to change. The change is the above paragraph.
%%%%%%%%

% We proceed with error detection for a single $\sigma$ as follows.  First, we compute $\upsilon_X$, i.e., $(h_{t_i}(\bar{x}), h_{t_j}(\bar{x})) \in \upsilon_X$ satisfying $Q[\bar{x}]$ in \tempgraph, and by definition, matches not satisfying defined constant literals in $X$ are discarded.  Second, we check whether the corresponding $\delta(X)$ of $\upsilon_X$ lies within $\Delta$, i.e., $|h_{t_{s_2}}(\bar{x}) - h_{t_{s_1}}(\bar{x})| \in \Delta$.  If not, these matches in $\upsilon_X$ are removed.  Third, for the remaining matches $(h_{t_i}(\bar{x}), h_{t_j}(\bar{x}))$ in $\upsilon_X$, we check whether $(h_{t_i}(\bar{x}), h_{t_j}(\bar{x})) \models Y$.  Since $\sigma$ is in normal form, $Y$ either contains a constant literal $y_{t_i}.A = a$, or a variable literal $y_{t_i}.A = y_{t_j}.B$.  If $Y$ contains a constant literal, and  $(h_{t_i}(\bar{x}), h_{t_j}(\bar{x})) \not \models Y$ for $(h_{t_i}(\bar{x}), h_{t_j}(\bar{x})) \in \upsilon_{XY}$, then we add matches in $\upsilon_X$ to \errorsigma.  Alternatively, if $Y$ contains a variable literal, then we check whether matches in each $\upsilon_X$ correspond to different values in $Y$, and if so, an error exists.  For each $\upsilon_X$, there exists a $\delta(X)$ representing the time interval where the values in $X$ hold.  For each $\delta(X)$, there exists one or more intervals $\delta_{XY}$, corresponding to the time intervals where unique values in $XY$ hold.  If there exists a single $\delta(XY)$, i.e.,  $\delta(X) = \delta(XY)$, then there is no violation.  However, if a $\delta(X)$ `splits' into two or more intervals $\delta_i(XY), i \geq 2$, then a change in the $Y$ value has occurred at the time point between two intervals, leading to an violation.  Hence, we add the corresponding $(h_{t_i}(\bar{x}), h_{t_j}(\bar{x})) \in \upsilon_X$ to \errorsigma.

%\subsubsection{Constant Literals}
%Let where $X, Y$ contain constant literals of the form $x_{t_i}.A = a, y_{t_i}.C = c$, for constants $a, c$.We compute all matches ($h_{t_i}(\bar{x})$,  $h_{t_j}(\bar{x})$) of $Q[\bar{x}]$ in \tempgraph, and filter matches not satisfying the constant literal conditions in $X$.  For the set of accompanying intervals $\delta_i = [s_i, e_i]$, representing when the matches are valid, we check for each $\delta_i$ whether $|e_i - s_i| \in \Delta$.  If so, we check 
%whether ($h_{s_i}(\bar{x})$,  $h_{e_i}(\bar{x})$) $\models Y$, i.e., $h_{t_{i'}}({y}) = c, \forall t_{i'} \in \delta_i$.  
%For any matches where  $h_{t_{i'}}({y}) \neq c$, we add $h_{t_{i'}}({\bar{x}})$ to \errorsigma.



%\subsubsection{Variable Literals}
%Let $\sigma = (Q[\bar{x}],\Delta, X \rightarrow Y)$ where $X, Y$ contain variable literals of the form $x_{t_i}.A = z_{t_j}.B$.  This requires checking equality among node attribute values for each pairwise match.  Similar to the constant literal case, we compute all matches ($h_{t_i}(\bar{x})$,  $h_{t_j}(\bar{x})$) of $Q[\bar{x}]$ in \tempgraph, but we partition the set of matches $\mathcal{H}$ according to their node attribute values in $X$.  That is, let $\upsilon_X  = \{h_{t_i}(\bar{x}),  h_{t_j}(\bar{x}) | h_{t_i}({x}).A = h_{t_j}({x}).A, \forall A \in X\}$  represent a partitioning of $\mathcal{H}$ such that all matches in a partition $\upsilon_X$ share the same values for all attributes $A \in X$.  For  entities in $\upsilon_X$, the intervals $\delta_i$ correspond to when the values are valid.  To verify the temporal conditions of $\sigma$, we check whether the validity period of the values lie within $\Delta$, i.e., $|\delta_i| = |e_i - s_i| \in \Delta, \forall i$.  We discard  matches that lie outside of $\Delta$. 


\begin{example}
\newText{ Following Example~\ref{ex:singleTGFD1}, we capture $e_1$ and $e_2$ by using graph pattern $Q_1[\bar{x}]$. $\upsilon_{X_{21}}$ is the match of the player $e_2$, which has no change from \lit{Sep. 2019} to \lit{Apr. 2020} and is shown on Figure~\ref{fig:TEDexample}(b). 
%\fei{Where is this seen in Fig 5 exactly?} 
If we compute $\delta(X_{21}Y_1)$, it has only one time interval as $[Sep.2019,Apr.2020]$ and since it doesn't lie within $\Delta=(0,6 months)$, we remove $\upsilon_{X_{21}}$. However, for we have two time intervals $\delta(X_{11}Y_1)$ and $\delta(X_{11}Y2)$, which split $\delta(X_{11})$ and both lie within $\Delta$. Therefore, we add $\upsilon_{X_{11}}$ to \errorsigma. One can verify that $\upsilon_{X_{12}}$ and its corresponding time interval $\delta(X_{12})$ has only one $\delta(X_{11}Y_1)$, which doesn't lead to any violation.  %\fei{How about discarding matches not satisfying constant literals?}\morteza{I had the other pattern for just constant literals, where you asked to remove. Do I have to add it again?}\fei{It was more about having a $\sigma$ that had constant and variable literals together as the text describes discarding matches not satisfying constant literals, and then moving on to check variables.  I think the previous version had *only* constant literals, we are now combining variables and constant literals together to be more general.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\fei{I don't think you need (p,q) in the variable list.  $p,q$ is used for the interval and should not be confused with $p1$ for player, confusing.}
% Let $\sigma'=Q_2[p,q,w,x,y,z]=(0,6\ months),  (x_{t_i}=x_{t_j} \land w_{t_i}=w_{t_j} \land z_{t_i}=z_{t_j} \rightarrow y_{t_i}=y_{t_j})$ \fei{Why do we have = interval?}  with $Q_2$ of Figure~\ref{fig:TEDexample}(b). $\sigma'$ imposes that any two matches of \lit{soccer players} with the time difference of $(0, 6\ months)$, if they have the same \lit{name} and play in the same \lit{team} and \lit{league} (\emph{i.e., the same player}), then they should have the same \lit{squad number}. This comes from the fact that the soccer players can only change their squad numbers at the pre-season and mid-season in \lit{La Liga}. In \tempgraph of Figure~\ref{fig:TEDexample}(a), there are two players at each timestamps that match $Q_2$, but we can only pair the matches that satisfy $\Delta$. Hence, we have the partition set as $\upsilon_{X_1}  =\{(h_1(p_1),h_2(p_1)),(h_2(p_1),h_3(p_1))\}$and $\upsilon_{X_2}  =\{(h_1(p_2),h_2(p_2)),(h_2(p_2),h_3(p_2))\}$, where $X_1$ (resp. $X_2$) is the equality of attributes for the player $p_1$ (resp. $p_2$) and $h_i(p_j)$ is the match of $p_j$ at time $t_i$. Now, if we compute $\upsilon_{X_2Y_2}$, it equals to  $(h_2(p_2),h_3(p_2))$, where we miss one valid pair $(h_1(p_2),h_2(p_2))$ and this is a violation.
As another example, consider $\sigma' = Q_2[x,y,z], (0,12\ months), (x_{t_i}=``Real Madrid CF" \land z_{t_i}=z_{t_j} \rightarrow y_{t_j}=``White")$, where $Q_2[\bar{x]}$ is depicted in Figure~\ref{fig:TEDexample}(a). $\sigma'$ enforces that if the team \lit{``Real Madrid''} plays in any league for one year, the \lit{``Home kit color''} of the team has to be \lit{``White''}. Using the graph of Figure~\ref{fig:TEDexample}(a), the $\upsilon_{X'_{1}}$ of the match $Real\_Madrid$ has the corresponding time interval $\delta(X'_{1})=[Sep.2019,Apr.2020]$. However, $\upsilon_{X'_{1}}$ splits into two $\upsilon_{X'_{1}Y'_1}$ and $\upsilon_{X'_{1}Y'_2}$ with time interval $\delta(X'_{1}Y'_1)=[Sep.2019,Nov.2019]$ and $\delta(X'_{1}Y'_2)=[Dec.2019,Apr.2020]$ resp, where both of them lie within $\Delta$. Since $Y$ of the $\sigma'$ has only constant literal, we have to simply check whether $\upsilon_{X'_{1}Y'_1}$ and $\upsilon_{X'_{1}Y'_2}$ satisfy $Y$. Based on this, $\upsilon_{X'_{1}Y'_2}$ violates $\sigma'$ and will be added to  \errorsigma.
}
\end{example}

% \fei{I think your figure example needs to use time points to show the timeline and we can refer to the time between time points as intervals.  For your purposes, this will require you to show actual time points (month of year) when a value is valid (both the start and end time point) of each value so it's clear when a change occurs.  I am trying to sync my previous figure with yours, but not sure how your example will unfold.}

%\fei{I think the last sentence misses the point of how to compute the errors. We should be using the intervals to help us identify when a change occurs from  $\upsilon_{X}$ to $\upsilon_{XY}$, as if there is more than one $\delta_i$ interval, then there are distinct $Y$ values.  We should be using the $\delta$ intervals to make this point, not the matches.  Same with the previous example.} 

% \fei{Morteza: please consolidate Example 7 and 8 into a single example, and update as per our discussion on Jan 8th to reflect the intervals.  You can simplify and use a TGFD with constant and variable literals.}
% \begin{example}
% \newText{Figure~\ref{fig:TEDexample}(a) shows a temporal graph \tempgraph over timestamps $t_1$ to $t_3$. The changes in the \tempgraph in each timestamp is provided in red while the unchanged attributes are emitted. Let $\sigma=Q_1[p,q,w,x,y,z]=(0,1\ year), (x_{t_i}=``Toni\ Kroos" \land w_{t_i}=``La\ Liga" \land z_{t_i}=``Real\ Madrid\ CF" \rightarrow y_{t_j}=``White")$, where $Q_1$ is depicted in Figure~\ref{fig:TEDexample}(b). $\sigma$ imposes that any two matches of the soccer player named \lit{Toni Kroos} who plays in the team \lit{Real Madrid CF} in \lit{La Liga} with the time difference of 0 to 1 year, should have the home kit color as \lit{White}. There are three matches $h_1$, $h_2$ and $h_3$ of $Q_1$ on the player $p_1$ over timestamps $t_1$, $t_2$ and $t_3$ resp. The valid pairs are $\{(h_1,h_2),(h_1,h_3),(h_2,h_3)\}$ with accompanying intervals as $\delta_{X}=\{[t_1,t_2],[t_1,t_3],[t_2,t_3]\}$. All three valid pairs satisfy $X$, while $(h_1,h_3)\not\models Y$ and $(h_2,h_3)\not\models Y$ since $h_3$ has $y_{t_3}=``Pink"$. Hence we add $h_3$ to \errorsigma.} 
% \end{example}



\subsubsection{Algorithm.}
\newText{ Pseudo code of \tedsingle is shown as Algorithm\ref{alg:singleTED}. Let \tempgraph \ and $\sigma= (Q[\bar{x}],\Delta, X \rightarrow Y)$ be the input. The output is all the set of violations of $\sigma$ in \tempgraph \ as \errorsigma. After initialization, we set $\cal{H}$ to be all the matches of $Q[\bar{x}]$ in the \ \tempgraph and compute $\upsilon_X$ and $\delta(X)$ for each match (lines 2-3). Then, we analyze every pair of matches in $\upsilon_X$. We compute $\upsilon_{XY}$ and $\delta(XY)$ corresponding to each $\upsilon_X$ (Line 5). Then, we remove any pair of matches that its time interval $\delta(XY)$ that doesn't lie within $\Delta$ (Lines 7-8). If the time interval lies within $\Delta$ and $Y$ only contains constant literals, we simply check whether the match satisfy $Y$ to find violation (Lines 9-10). After computing all the matches in $\upsilon_{XY}$ and remove those that do not lie within $\Delta$, if we have variable literal in $Y$, we simply check if $\delta(X) \neq \delta(XY)$ to find violation (lines 11-13). 
%If $\sigma$ has only constant literals, we pair all the matches from $\cal{H}$ such that their time difference lies within $\Delta$. If so, we check whether they satisfy $X$ and not satisfy $Y$. Such pairs will be considered as violation and added to \errorsigma \ (lines 3-7). If $\sigma$ has variable literals, for every pair of matches, if they lie within $\Delta$ and satisfy the constant literals in $X$, then we add the pair to the corresponding partition $\upsilon_X$ based on the variable literals in $X$ (lines 9-11). Then, for each partition $\upsilon_{X_i} \in \upsilon_X$, we compute $\upsilon_{X_iY_j}$ given the variable and constant literals in $Y$ (lines 12-13). If $\upsilon_{X_iY_j}\neq \upsilon_{X_i}$, then it means either the corresponding time interval has been violated in $Y$ or it has been split to more than one time interval, which is a violation and the pairs in $\upsilon_{X_i}$ will be added to \errorsigma (lines 14-15). 
At the end, we return \errorsigma.}

\input{Algorithms/alg1new2.tex}

==> summarization.tex <==
\subsection{Optimizations}

\fei{Old text for now.}
\subsubsection{Pattern Overlap and Clustering}
If we extend the single \tgfd case for a set of \tgfds $\Sigma$, a naive solution computes matches of the graph pattern $Q[\bar{x}]$ against \tempgraph \ for each $\sigma \in \Sigma$.  This solution becomes infeasible for large \tempgraph.  

We propose a solution that exploits the \emph{structural} and \emph{spatial} locality among the graph patterns in $\Sigma$.  For a set of graph patterns $\mathcal{Q}= Q_i[\bar{x}]$, $i = \{1 \ldots |\Sigma|\}$, we seek to cluster nodes that are of equal type and share the same topology.  We construct a graph \latentgraph that draws a latent edge between nodes from each pair of graph patterns $Q_i[\bar{x}]$ to achieve connectivity.  

We address this problem as a graph summarization problem with the goal of transforming \latentgraph to a \emph{summary graph}, \summarygraph, consisting of \emph{super nodes} and \emph{super edges}.  Super nodes cluster vertices in \latentgraph  of the same type, and super edges represent references between different types of nodes.  Formally, let \latentgraph $= (V_{\mathcal{Q}}, E_{\mathcal{Q}})$, where  $V_{\mathcal{Q}}$ are nodes with a \texttt{type} from patterns in $\mathcal{Q}$, and $E_{\mathcal{Q}}$ represent the set of directed edges from $\mathcal{Q}$.  We define  $V_{\mathcal{Q}}$ and $E_{\mathcal{Q}}$ as \emph{simple nodes} and \emph{simple edges}, respectively, from \latentgraph, and a directed edge pointing to a simple node. 

Let \summarygraph = $(V_S, E_{S})$, denote a summary graph consisting of super nodes $V_S$ that cluster simple nodes from \latentgraph \ into similar types.  Let $E_{S}$ denote super edges that connect two super nodes $v_1, v_2 \in V_S$.  
Note that super nodes and super edges include the set of simple nodes and simple edges, respectively, in cases where the topological or clustering criteria are not met.  For example, a node of type $A$ may be excluded from the super node clustering of other type $A$ nodes due to having a different subgraph topology.  Figure~\ref{fig:graphPatterns}(a) shows this case where $Q_3[\bar{x}]$ shows that node $A$
 does not share the same structural topology with node $B$ as the other two patterns $Q_1[\bar{x}]$and $Q_2[\bar{x}]$.  

\eat{ 
\textbf{Objective Function.}
We construct \summarygraph by aggregating nodes of the similar type to a super node.  We adopt a similar philosophy to entity resolution based summarization algorithms that a good summarization requires nodes in a super node to be equivalent (or highly similar)~\cite{ZhuGSGK16}.  Given this node similarity, we expect that connections from these coherent nodes to share similar connections to other super nodes, i.e., achieving structural similarity.  This intuition leads to maximize similar connectivity patterns across coherent nodes.  To achieve coherence among nodes, we use an objective function that clusters similar type nodes according to a similarity function $sim()$~\cite{ZhuGSGK16}: 

\begin{equation}
    argmax \sum_{k} \sum_{v_1, v_2 \in V_k} sim(v_{1}', v_{2}') 
\end{equation}

For structural similarity, we seek maximum common subgraphs shared among the graph patterns in $\mathcal{Q}$.  A super edge connects two super nodes $v_1, v_2 \in V_S$, and a simple edge $e(v_{1}', v_{2}') \in E_{S}$ connects nodes $v_{1}', v_{2}'$ where, without loss of generality, $v_{1}'$ (or $v_{2}'$) is a simple node, i.e.,  $v_{1}'$ (or  $v_{2}'$) $\in V_{\mathcal{Q}}$.
\fei{This needs some more thought on complexity, criteria and trade-off with coherence (spatial similarity).}
}

\begin{example}
Figure~\ref{fig:graphPatterns}(a) shows three graph patterns $\{Q_{1}[\bar{x}], Q_{2}[\bar{x}], Q_{3}[\bar{x}]\}$, associated with \tgfds $\{\sigma_1, \sigma_2, \sigma_3 \} \in \Sigma$.  To maximize spatial and structural locality, we cluster nodes of maximum similarity (of equal type), and identify maximum common subgraphs among the graph patterns, denoted as red, blue, and black outlines.  Figure~\ref{fig:graphPatterns}(b) shows a summary graph with super and simple nodes denoted as shaded and non-shaded nodes, respectively.  Super edges and simple edges are represented as solid and dashed lines, respectively.  Each edge is associated with a label stating which \tgfds include the participating nodes in their respective graph patterns. 
\end{example}

\begin{figure}[tb]
	{\includegraphics[scale=0.345]{figures/sec5_patterns_graphs.png}}
	\vspace{-1ex}
	\caption{(a) Example graph patterns; (b) Summary graph.}\label{fig:graphPatterns}
	\vspace{-1ex}
\end{figure}

While our work is amenable to any graph summarization algorithm, we use the \texttt{CoSum} algorithm in our implementation~\cite{ZhuGSGK16}.  In the next section, we describe how we use the summary graph \summarygraph to retrieve matches for each $\sigma \in \Sigma$. 

%\fei{Describe algorithm to compute your dependency graph for patterns, via graph summarization methods as per survey as a starting point.  Some starting points to think about: input graph can be directed, and method should consider heterogeneous, node(edge) grouping based method that produces weighted edges.}

\subsubsection{Computing Connected Components}
We seek an ordering to traverse the super nodes in \summarygraph. For a visited super node $v_1 \in V_S$, let $v_1.\texttt{att}$ denote a node property (attribute).  We retrieve matches satisfying the literals $x \in X$ for each $\sigma$ where $v_1.\texttt{att} \in X$.  We seek an ordering such that for each subsequent visit to node $v_2$ (after $v_1$), our working set of matches are those that satisfy the literals w.r.t. $\{v_1.\texttt{att}, v_2.\texttt{att} \} \in X$ for a maximal number of $\sigma \in \Sigma$. 

Since \summarygraph \ may contain cycles, we first compute the strongly connected components of \summarygraph, which is guaranteed to be a directed acyclic graph (DAG).  We use the \emph{Tarjan algorithm} to compute the strongly connected components, which runs in time $O(V_S, E_{S})$~\cite{CLR}.   For each connected component \component, we topologically sort the nodes, which can be done in time $O(V_S + E_S)$.

The topological sorting induces a node ordering which for each visited node $v_1$, and subsequent node $v_2$ retains matches $h_1(\bar{x}), h_2(\bar{x})$ from the working set satisfying attributes $v_1.\texttt{att}$ and $v_2.\texttt{att}$.


\eat{
\textbf{Special Cases.}
\begin{itemize}
    \item Let $\sigma = (Q[\bar{x}],\Delta, X \rightarrow Y)$, $\sigma' = (Q'[\bar{x}],\Delta', X' \rightarrow Y')$, such that $Q' \subseteq Q$.  If ($h_{1}(\bar{x})$,  $h_{2}(\bar{x})$)  $\models X'$ over $\Delta'$, then ($h_{1}(\bar{x})$,  $h_{2}(\bar{x})$) $ \models X$, for $X = X', \Delta \subseteq \Delta'$.  %just a variant of interval containment axiom
  %  \item Let $\sigma, \sigma'$ be defined as above, but with $X' \subseteq X$,  $\Delta' \subseteq \Delta$, and $Y = Y'$.  If \tempgraph $\not \models \sigma$, then \tempgraph $\not \models \sigma'$, and we can directly eliminate the verification checking for $\sigma'$.  %fei: don't think 2nd case is true.
\end{itemize}
}


